Generative AI for Secure Physical Layer Communications: A Survey

Generative Artificial Intelligence (GAI) stands at the forefront of AI innovation, demonstrating rapid advancement and unparalleled proficiency in generating diverse content. Beyond content creation, GAI has significant analytical abilities to learn complex data distribution, offering numerous opportunities to resolve security issues. In the realm of security from physical layer perspectives, traditional AI approaches frequently struggle, primarily due to their limited capacity to dynamically adjust to the evolving physical attributes of transmission channels and the complexity of contemporary cyber threats. This adaptability and analytical depth are precisely where GAI excels. Therefore, in this paper, we offer an extensive survey on the various applications of GAI in enhancing security within the physical layer of communication networks. We first emphasize the importance of advanced GAI models in this area, including Generative Adversarial Networks (GANs), Autoencoders (AEs), Variational Autoencoders (VAEs), and Diffusion Models (DMs). We delve into the roles of GAI in addressing challenges of physical layer security, focusing on communication confidentiality, authentication, availability, resilience, and integrity. Furthermore, we also present future research directions focusing model improvements, multi-scenario deployment, resource-efficient optimization, and secure semantic communication, highlighting the multifaceted potential of GAI to address emerging challenges in secure physical layer communications and sensing.

==> Application.tex <==
\section{Application Layer}

\subsection{Problems}

\begin{itemize}
    \item \textbf{Anonymization}:

    
\end{itemize}



\subsection{Traditional AI methods}




\subsection{Generative AI methods}

ZipNet-GAN: Inferring finegrained mobile traffic patterns via a generative adversarial neural network


\cite{sun2023disentangled} disentangled information bottleneck guided privacy-protective jscc for image transmissio
In this paper, we propose a disentangled information bottleneck guided privacy-protective JSCC (DIB-PPJSCC) for image transmission, which aims at protecting private information and achieving superior communication performance

==> Augmentation.tex <==
\section{Data Reconstruction and Augmentation}\label{sec:data}

\begin{table*}[htp] \scriptsize%\footnotesize
  \centering
  \caption{Summary of GAI for Data Reconstruction and Augmentation in Physical Layer}
  \label{tab:data}
    \begin{tabular}{m{0.11\textwidth}<{\centering}||m{0.06\textwidth}<{\centering}|m{0.09\textwidth}<{\centering}|m{0.64\textwidth}<{\centering}}
      \hline
      \textbf{Techniques}  &  \textbf{Reference} & \textbf{Algorithm} & \textbf{Pros \& Cons} \\
       \hline
        \multirow{5}{0.11\textwidth}[-25pt]{\centering Data Reconstruction} & \cite{tran2018generative}  & SARGAN & \begin{itemize}[leftmargin=*]
        \item[\textcolor{blue-green}{\ding{108}}] A GAN network to recover this missing spectral information
        \item[\textcolor{green}{\ding{51}}] Not require any information of the missing band locations
        \item[\textcolor{green}{\ding{51}}] All computational complexity is at the training phase. 
        \item[\textcolor{red}{\ding{55}}] The requirement for extensive training data
        \vspace{-1.0em}
        \end{itemize}\\
        \cline{2-4}
    & \cite{feng2022waveform}  & VAE-GAN  & \begin{itemize}[leftmargin=*]
    \item[\textcolor{blue-green}{\ding{108}}] A VAE-GAN-based method for reconstructing DSSS signals
      \item[\textcolor{green}{\ding{51}}] Avoid complex parametric analysis of the signal
      \item[\textcolor{green}{\ding{51}}] Integrate DRSNs and self-attention in VAE-GAN
      \item[\textcolor{red}{\ding{55}}] Unsatisfactory effect in low SNR
      \vspace{-1.0em}
      \end{itemize}\\
      \cline{2-4}
    & \cite{guo2023high}  & MTS-GAN& \begin{itemize}[leftmargin=*]
    \item[\textcolor{blue-green}{\ding{108}}] A high-precision reconstruction method for electromagnetic environment data based on MTS-GAN
        \item[\textcolor{green}{\ding{51}}]  Use the GRUI to simulate time irregularities
      \item[\textcolor{green}{\ding{51}}]  High accuracy and convergence speed
      \item[\textcolor{red}{\ding{55}}] The specific requirements for training and implementing
      \vspace{-1.0em}
      \end{itemize}\\
      \cline{2-4}
            &  \cite{estiri2020variational} & VAE & \begin{itemize}[leftmargin=*]
            \item[\textcolor{blue-green}{\ding{108}}]  Investigate the performance of VAEs and compare the results with standard AEs
          \item[\textcolor{green}{\ding{51}}]  Use SSIM metric instead of the peak signal-to-noise ratio
      \item[\textcolor{red}{\ding{55}}] Limited in terms of the variety of noise models
      \vspace{-1.0em}
      \end{itemize}\\
      \cline{2-4}
     & \cite{wu2023cddm}  & CDDM & \begin{itemize}[leftmargin=*]
     \item[\textcolor{blue-green}{\ding{108}}] A channel denoising diffusion models for wireless communications to eliminate the channel noise
          \item[\textcolor{green}{\ding{51}}] Eliminate the channel nosie under Rayleigh fading channel and AWGN channel
      \item[\textcolor{red}{\ding{55}}] Relatively long sampling time
      \vspace{-1.0em}
      \end{itemize}\\
      \hline
      \multirow{4}{0.11\textwidth}[-10pt]{\centering Data Augmentation} & \cite{davaslioglu2018generative}  & SAGA (Class) & \begin{itemize}[leftmargin=*]
      \item[\textcolor{blue-green}{\ding{108}}] An approach of training data augmentation and domain adaptation for cognitive radio
          \item[\textcolor{green}{\ding{51}}] Achieve both data augmentation and domain adaptation
      \item[\textcolor{red}{\ding{55}}]  Instability in GAN training
      \vspace{-1.0em}
      \end{itemize}\\
      \cline{2-4}
      & \cite{tang2018digital} & ACGAN (Class) & \begin{itemize}[leftmargin=*]
      \item[\textcolor{blue-green}{\ding{108}}] An approach to programmatic data augmentation method by using ACGANs
          \item[\textcolor{green}{\ding{51}}] Introduce several tricks in GAN training
      \item[\textcolor{red}{\ding{55}}]  Relatively long training time
      \vspace{-1.0em}
      \end{itemize}\\
      \cline{2-4}
     &\cite{roy2019generative}  &  WGAN-GP (Spoofing) & \begin{itemize}[leftmargin=*]
     \item[\textcolor{blue-green}{\ding{108}}]  The task of full-band spectral generation in addition to single signal generation 
          \item[\textcolor{green}{\ding{51}}] Treat LTE signals as 2D images
      \item[\textcolor{red}{\ding{55}}] Poor performance of generated signals
      \vspace{-1.0em}
      \end{itemize}\\
      \cline{2-4}
      &\cite{lu2021gan} & MSGAN (Detection) & \begin{itemize}[leftmargin=*]
      \item[\textcolor{blue-green}{\ding{108}}] A domain-specific framework consisting of offline training and online inference to detect anomalies in the scenario of industrial robotic sensors
      \item[\textcolor{green}{\ding{51}}]  Use an adaptive update strategy during offline training
      \item[\textcolor{red}{\ding{55}}] Lack of analysis that extends to diversity scenarios
      \vspace{-1.0em}
      \end{itemize}\\
      \hline
    \end{tabular}
\end{table*}

In communications and signal processing, different systems often operate within the same or overlapping frequency bands \cite{musaloiu2008minimising}. This overlap often leads to the spectral information from one system interfering with or being confounded by that of another. Such interference can introduce noise and inaccuracies in the received signals, potentially resulting in reduced usable data \cite{gummadi2007understanding}. To mitigate these challenges, two primary approaches are employed: data reconstruction and data augmentation, by respectively restoring corrupted signals to their original state and introducing additional synthesized data to provide a more robust and diverse dataset.

\subsection{Data Reconstruction}

Data reconstruction focuses on retrieving the original signal or information from corrupted or incomplete  datasets \cite{chai2020deep}. This process involves various techniques to restore or approximate the original data, aiming to overcome the issues caused by interference and noise. Data augmentation, on the other hand, is centered on generating additional usable data from the limited existing dataset. It involves applying transformations or manipulations to enhance the features of the existing data, thereby expanding the dataset. This expansion is crucial for improving data analysis and model training, particularly in scenarios where the amount of collected data is inherently limited.

Traditional reconstruction methods, based on sparse representation and low-rank matrix completion \cite{wei2010sparse, nguyen2014sparse}, assume that both full-spectrum data and their corrupted counterparts are sparsely represented with a full-spectrum and a gapped-spectrum dictionary, respectively. Therefore, both representations are similarly sparse and share identical sparse codes. Consequently, these reconstruction methods lack the ability and robustness to distinguish closely situated targets at high resolution accurately without prior knowledge of the missing frequency bands. However, GAI models excel in learning complex data patterns. GAI models are particularly adept at generating and reconstructing data, effectively reducing the dependency on prior knowledge of missing frequency bands. Moreover, GAI models leverage their advanced learning capabilities to data gaps, offering a more robust and flexible approach to signal reconstruction.

In \cite{tran2018generative}, the authors introduced a GAN framework named SARGAN, designed to reconstruct missing spectral information in Ultra-wideband (UWB) radar systems across multiple frequency bands. Specifically, SARGAN focuses on recovering Synthetic Aperture Radar (SAR) data \cite{moreira2013tutorial}. To train the GAN model, the model uses numerous data pairs, each comprising an uncorrupted scene and its frequency-corrupted version. The corrupted datasets are simulated by removing random frequency bands from the original data. A significant advantage over conventional spectral recovery methods is that the proposed model does not need any prior knowledge of the missing data. This is particularly beneficial in unpredictable scenarios including battlefield conditions, where jamming and interference can occur unexpectedly. The simulation results show that the recovered signals using SARGAN achieve an average gain of over 18 dB in signal-to-noise ratio, even when up to 90\% of the operating spectrum is missing.

Compared to radar data, Direct Sequence Spread Spectrum (DSSS) signals possess more complex structures. This complexity makes it challenging to characterize accurately the properties of a target signal using traditional methods. To extract more properties such as Pseudonoise (PN) sequence \cite{helleseth2021pseudo}, a method based on VAE-GAN \cite{larsen2016autoencoding} for reconstructing DSSS signals was proposed in \cite{feng2022waveform}. By integrating VAE and GAN, the encoder provides the generator with a loss function that measures the discrepancy between real and generated data. This integration contributes to enhanced stability of the network during the training process. Furthermore, the proposed framework incorporates a Deep Residual Shrinkage Network (DRSN) \cite{zhao2019deep, jiang2022image} and a self-attention mechanism \cite{vaswani2017attention} into the encoder and discriminator. The DRSNs are effective in minimizing redundant information in the collected signal, particularly noise-induced redundancy. Meanwhile, the self-attention mechanism facilitates the establishment of long-distance dependencies within the input sequences. However, while the proposed model is adaptable to PN sequences with varying code lengths, its performance in low Signal-to-Noise Ratio (SNR) environments significantly diminishes. Particularly, when the SNR falls below 13 dB, there is a sharp decline in the model's performance \cite{feng2022waveform}.

\begin{figure}[htp]
    \centering
    \includegraphics[width= 0.95\linewidth]{figs/Constru2.pdf}
    \caption{The MTS-GAN data completion network structure \cite{guo2023high}. The generator network is built by the gated loop unit GRUI for data interpolation. GRUI can simulate time irregularities allowing for more accurate extraction of the distribution characteristics of time-frequency signal data.}
    \label{fig:constru}
\end{figure}

To improve the precision of reconstructing electromagnetic environment data, the authors in \cite{guo2023high} developed a high-precision method using a Multi-Component Time Series Generation Adversarial Network (MTS-GAN). This approach effectively utilizes multivariate time series data to better capture the correlations between the time and frequency domains of electromagnetic data (Fig \ref{fig:constru}). A key component of this method is the use of a Gate Recursive Unit (GRUI), which simulates time irregularities. The GRUI allows for more accurate extraction of the distribution characteristics of time-frequency signal data and reduces the impact of random losses in time series. The proposed method achieves high accuracy and ensures rapid convergence and iterative optimization speeds with the 'Qingdao Offshore Measurement Data Set' \cite{guo2023high}.

Besides GANs, VAEs are recognized as another powerful GAI model for effective data reconstruction. In \cite{estiri2020variational}, a VAE-based model was proposed for data construction in noisy channels. The AE and VAE models are particularly effective in regularizing the latent space distribution, a feature that is highly beneficial in data reconstruction with Gaussian noise channels. However, traditional AEs \cite{bourtsoulatze2019deep} perform poorly, particularly under low SNR conditions. In such environments, data points in the latent space can undergo random deviations from their original positions. In contrast, the VAE's regularized latent space facilitates accurate decoding by the decoder, thus improving performance in noisy settings. Consequently, when evaluated on the STL10 dataset \cite{coates2011analysis} using the Structural Similarity Index (SSIM) metric \cite{brunet2011mathematical}, the VAE-based method demonstrates a smoother output attributed to its inherent structure.

DMs have garnered attention in the field of wireless communications due to their inherent ability to progressively remove noise, especially in aiding receivers to mitigate channel noise. In response to this potential, the study \cite{wu2023cddm} introduced Channel Denoising Diffusion Models (CDDM) specifically designed for wireless communications. CDDM aims to leverage the noise reduction properties of DMs to enhance the quality and reliability of signal reception in wireless communication channels. CDDM is trained using a specialized noise schedule specifically adapted to the wireless channel, enabling the effective elimination of channel noise through sampling algorithm. The training algorithm for the combined CDDM and JSCC system is structured into three distinct stages. In the first and last stages, the JSCC encoder and decoder are trained to minimize the reconstruction error. The second stage involves fixing the parameters of the JSCC encoder, thereby allowing the CDDM to learn the distribution of latent representations. This stage utilizes a noise schedule that closely simulates the distribution of channel noise, rendering the CDDM adaptable to a variety of channel conditions. The results demonstrate that systems  incorporate CDDM consistently outperform those without CDDM across all SNR regimes, under both AWGN and Rayleigh fading channels. Notably, under an AWGN channel and a Rayleigh fading channel at 20 dB SNR, the CDDM achieves a 0.49 dB gain and 1.06 dB gain respectively \cite{wu2023cddm}.


As summarized in Table \ref{tab:data}.
In summary, the application of GAI in data reconstruction showcases its remarkable ability to process and regenerate missing or corrupted data, ensuring integrity and continuity in noisy channels. Utilizing techniques such as GANs and VAEs, GAI aids in the restoration of compromised data and enhances the resilience of systems by improving the quality and reliability of the reconstructed data.

\subsection{Data Augmentation}

As deep learning techniques become increasingly integrated into secure physical communication and sensing, there is a pronounced need for extensive training data to capture the intricate dynamics of spectrum, channels, and emitters \cite{jeon2023advanced}. However, a training dataset of all potential spectrum conditions is often prohibitively expensive and impractical. This challenge is exacerbated by the fact that an extended period of spectrum sensing for data collection will severely limit the available time for actual data transmission \cite{wang2023generative}. Furthermore, changes in the spectrum environment necessitate the collection of new training data for retraining classifiers. Classifiers trained with outdated data may not yield reliable results under new conditions, as the previous training data might not accurately represent the characteristics of the new test environment \cite{roh2019survey}. This discrepancy can lead to inaccuracies and inefficiencies in the classification process. Given these challenges, there is a clear need for data augmentation to enhance the training process. GAI models are particularly well-suited for this task. They can effectively augment data by generating synthetic samples that mimic real-world conditions, thereby enriching the training dataset and improving the robustness and adaptability of classifiers to varying spectrum environments \cite{li2019enhanced}.



\begin{figure}[htp]
    \centering
    \includegraphics[width= 0.95\linewidth]{figs/Aug3.pdf}
    \caption{Proposed SAGA architecture \cite{davaslioglu2018generative}. 
    In \textit{Part A}, C-GAN is deployed to learn and generate spectrum data with labels to enhance the training dataset at given spectrum environment.
    \textit{Part B} illustrates the Data Adaptation, where a bidirectional GAN, through an inverse mapping process, assists in adapting the labels from the old environment to train the CGAN in the new environment.
    }
    \label{fig:aug}
\end{figure}


In spectrum sensing, the aim is to detect the presence of an emitter based on spectrum data, where the channel conditions and emitter features often change and are unknown. Traditional methods such as the energy detector \cite{axell2012spectrum} could not achieve satisfactory results since they depend greatly on these changing conditions. To address these challenges, \cite{davaslioglu2018generative} introduced Spectrum Augmentation/Adaptation with a Generative Adversarial Network (SAGA) (Fig \ref{fig:aug}). SAGA employs C-GAN \cite{mirza2014conditional} to learn and generate realistic spectrum domain data with labels to enhance the training dataset at given spectrum environment. Furthermore, SAGA demonstrates a notable capacity for adapting to new spectrum environments where labeled training data is unavailable. It combines a bidirectional GAN \cite{donahue2016adversarial}, a CGAN, and a classifier. Through an inverse mapping process, the bidirectional GAN assists in adapting the labels from the old environment to train the CGAN in the new environment. Subsequently, a new classifier is trained with domain-adapted samples. Significantly, due to this domain adaptation mechanism, SAGA also shows potential for application in wideband spectrum sensing with multiple channels available.

Similarly, the authors in \cite{tang2018digital} concentrated on enhancing digital signal modulation recognition and introduced a data augmentation framework utilizing an improved C-GAN, known as ACGAN \cite{odena2017conditional}. The dataset employed in their study consists of eight categories of modulated signals: BPSK, 4ASK, QPSK, OQPSK, 8PSK, 16QAM, 32QAM, and 64QAM \cite{Peng2023DeepLearning}. These class labels are used to determine the specific type of Contour Stellar Image to be generated in the proposed framework. The experiments demonstrate that the proposed framework effectively enhances existing CNN classification algorithm in \cite{Peng2023DeepLearning}, improving the accuracy from 0.1\% to 6\% \cite{tang2018digital}.

In the realm of attack and defense strategies within wireless communications, simulating and imitating Radio Frequency (RF) signals is a basic tactic employed by jammers, spoofers, and other forms of attack. While GAI has demonstrated effectiveness in augmenting short time series segments, challenges remain in accurately generating RF signals, such as the length of signals, and radio environments \cite{roy2019generative}. The authors in \cite{roy2019generative} explored the potential of GAN models to accomplish full-band spectral generation, in addition to the generation of single signals. They implement the WGAN-GP model \cite{arjovsky2017wasserstein} to improve training stability, repeatability, and predictability. Drawing on its proven effectiveness in the image domain, they utilize spectral representations of OFDM signals called LTE \cite{ndujiuba2015comparative}, treating them as 2D images. Nonetheless, the study shows that using GANs to create long sequences over time is quite challenging. It is harder to capture small details and features in these long sequences than in the shorter ones\cite{roy2019generative}. 

In physical layer sensing, sensor failures within industrial systems can lead to significant operational disruptions, escalating production costs, or even catastrophic outcomes. This situation underscores an urgent need for effective technologies that accurately detect anomalies. A primary challenge in this area is the large amount of of unclean and irrelevant data collected from sensors, known as data imbalance \cite{thabtah2020data}. This issue often results in conventional AI models misclassifying all samples as abnormal, further complicating anomaly detection \cite{lee2021gan}. To tackle the data imbalance problem, \cite{lu2021gan} introduces the MSGAN model, a GAN-based data augmentation strategy specifically designed for sensor anomaly detection. This model integrates WGAN-GP \cite{arjovsky2017wasserstein} with a novel adaptive update strategy during offline training. The adoption of an adaptive update strategy allows the MSGAN to accelerate training convergence and improve the quality of synthetic samples. In particular, simulation results demonstrate the significant impact of data imbalance on anomaly detection accuracy. To be more specific, with a 1:100 imbalance ratio, the accuracy of the LightGBM model is only 87.1\%. In contrast, by using the proposed model to increase the ratio to 1:1 leads to a marked improvement in accuracy, reaching 97.2\% \cite{lu2021gan}. 

As summarized in Table \ref{tab:data}.

Employing GAI for data augmentation, a robustness and reliability dataset will be enriched in various domains. By creating varied and extensive datasets, GAI technologies like GANs learn from a broader range of scenarios, improving their accuracy and robustness in various tasks, and addressing the challenge of limited or imbalanced datasets in diverse applications.



==> Case.tex <==
\section{Case Study}\label{CS}

\subsection{Framework}



==> Future.tex <==
\section{Future Direction}

==> Gaimethod.tex <==
\section{Generative AI-based Methods}\label{Gmeth}

In this section, we investigate two aspects: firstly, Adversarial Learning to enhance conventional AI-based classifiers via GAI; secondly, the attack detection methods employing GAI within vehicular networks.



%In this section, we discuss the applications of generative AI-based methods in preserving security.

\subsection{Adversarial Learning}

Adversarial attack is a specialized form of attack that targets AI-based detection systems built with neural networks. Adversarial attacks use data containing a small perturbation imperceptible to humans to affect the prediction results of neural networks. Since the attack are difficult for humans to distinguish, it makes neural networks particularly vulnerable under this kind of attack, especially in maintaining the security of vehicular networks. 

The role of data exchange and communication from sensors is foundational in vehicular networks. At the decision-making stage, this exchange enables vehicles to achieve a more comprehensive understanding of their surroundings, which is a crucial component for autonomous driving. Current autonomous driving systems, typically transmit this data to a neural network-based decision maker, which is vulnerable under adversarial attacks. Take Tesla \cite{endsley2017autonomous}, which relies on image data collected by cameras combined with computer vision algorithms to make autonomous driving decisions, as an example. According to the demonstration from the cybersecurity firm McAfee \footnote{https://www.mcafee.com/blogs/other-blogs/mcafee-labs/model-hacking-adas-to-pave-safer-roads-for-autonomous-vehicles/}, the researchers fooled the car’s Mobileye EyeQ3 camera system by subtly altering a speed limit sign on the side of a road with several adversarial stickers. These tiny piece of stickers made the MobilEye camera’s top prediction for the sign to be 85 mph instead of 35. This experiment highlights potential threats when the autonomous driving system suffers from adversarial attack via Spoofing or Data Injection within the vehicle network targeting camera images. Therefore, improving the robustness of AI-based methods against adversarial attacks on sensor data, such as images, radar, etc., is crucial for ensuring vehicular network security and safety.

Currently, there are two approaches to solving such problems with the assistance of GAI: Adversarial Purification and Adversarial Examples, from the attack data perspective and the training dataset perspective respectively.

\begin{itemize}
    \item \textbf{Adversarial Purification:} From the attack data perspective, Adversarial purification aims learn a purification model removing adversarial perturbation of data before feeding them into detection systems. Due to the powerful learning capability regarding data distribution of generative models, they can restore clean data from attacked data.
    
    \textit{GAN:} A common limitation of existing AI-based approaches is that many these defenses are only designed for specific attack patterns and are not effective against new attacks. To address this issue, the authors in \cite{samangouei2018defense} propose a framework, Defense-GAN, leveraging GAN to defend adversarial attacks. This framework is designed against both white-box and black-box attacks. Via learning the distribution of unperturbed images, Defense-GAN can find a close output to a given image which does not contain the adversarial perturbation before feeding them to the classifier. To demonstrate superiority over prior data-driven models, Defense-GAN is compared with the adversarial learning framework, Magnet \cite{samangouei2018defense}, on several datasets with four different neural network architectures classifiers and substitute models combinations. For the MINST dataset, Defense-GAN has about 90\% accuracy against  FGSM black-box attack across all classifiers, where the highest accuracy of Magnet is only 75.71\%. For the FGSM whitebox attack, the accuracy of Defense-GAN are all above 95\%, whereas MAGnet only has a maximum of 19.1\% \cite{samangouei2018defense}. These results highlight the ability of GAN as an adversarial purification algorithm to protect vehicular networks better than the AI-based method from a variety of different adversarial attacks.
    
    
    \textit{DMs:} One of the challenges in adversarial purification of vehicular networks is to preserve most of local details in the purified data. Inspired by Denoising Diffusion Probabilistic Model (DDPM) whose latent space has the same dimension of the original input data, the authors in \cite{wang2022guided} propose GDMP, a novel framework designed to eliminate adversarial perturbation of input data. During diffusion steps of DDPM \cite{wang2022guided}, attacked images are injected with Gaussian noises to submerge its adversarial perturbations which will be eliminated with Gaussian noises simultaneously during the denoising process. To tackle the aforementioned challenge, an additional guidance is utilized to retain consistency between the purified image and the original one, which can boost the purification performance when using a large number of diffusion steps. Compared to the conventional transfer-based method \cite{wang2022guided}, the accuracy of GDMP algorithm against Preprocessor-blind PGD attacks \cite{wang2022guided} on CIFAR-10 dataset improves by nearly 6\%, reaching 93.5\%. Its robustness accuracy improves by 20\% than conventional methods, achieving a rate of 90\%, while the highest accuracy of the state-of-the-art generative methods is only 85.45\% \cite{wang2022guided}. In the context of vehicular networks, the significance of GDMP is that it can effectively improve the robustness of the system against attacks while guaranteeing the accuracy of information communication, thus improving the security of the system.
    
    
    % Similarly, in \cite{yoon2021adversarial}, the authors propose a Denoising Score-Mathing (DSM) method based on DMs. Since the purification can be thought as denoising of the adversarial attacks, DSM leans the score function denoising the perturbed data. 
    
    % The authors in \cite{wu2022guided} argue that generating from random noises with the guidance of adversarial inputs leads DMs to better purification effects. They use ResNet-50 classifier and attain a robust accuracy of 89.62\%, very close to the results reported in \cite{wang2022guided}. 
    
    % About parameters, the authors in \cite{nie2022diffusion} theoretical discuss the diffusion timestep, an important design parameter in their diffusion purification method (DiffPure). Their theoretical analysis reveals that the noise needs to be high enough to remove adversarial perturbations but not too large to destroy the label semantics of purified images. They propose a theorem characterizing how the diffusion timestep affects the difference between the clean image and purified image obtained by DiffPure, providing guidance on setting a suitable timestep.
    

    
    \item \textbf{Adversarial Examples:} From the training dataset perspective, improving adversarial robustness aims to augment the training data of the classifier with adversarial examples. Due to the powerful generative capabilities of generative models, they are well-suited for generating additional adversarial examples relying solely on existing datasets.
    
    
    % In \cite{gowal2021improving}, the authors explore how generative models trained solely on the original training set can be leveraged to artificially improve adversarial robustness. They show that generative models allow adversarial training to go well beyond the current state-of-the-art methods.
    
    \textit{GAN:} 
    One of the disadvantages in conventional adversarial examples generation is that it focuses only on generating data based on existing datasets, limiting their ability to customize the generated perturbations specifically for classifiers network. To address this issue, the authors in \cite{lee2017generative} propose a framework called Generative Adversarial Trainer (GAT), utilizing the capabilities of GAN to optimize the classifier and generator networks simultaneously. While the generator network creates adversarial perturbations to deceive the classifier, the classifier network is simultaneously trained to correctly classify both original and adversarial images. During the process of adversarial learning, GAT can produce data targeting the vulnerabilities of the classifier. By using the image gradients, it can effectively enhance the classifier's robustness. When applied to the CIFAR-10 dataset for classification, GAT shows a remarkable 4-6\% improvement in accuracy, where other regularization techniques as Dropout, or Random Perturbation approximately 1-2\% performance improvement over existing baseline network \cite{lee2017generative}. The generation of adversarial examples for vehicular networks currently are not adequately tailored for emerging types of attacks. This framework underscores the potential of GAN targeted defense against adversarial attacks enhancing the robustness of discriminative AI methods.

    
    \textit{DMs:} 
    A fundamental constraint of AI-based methods is the necessity for large datasets, which are frequently unavailable for emerging cyberattacks on vehicular networks. Focusing on the adversarial robust classification of image data, the authors in \cite{ouyang2023improving}  propose the Contrastive-DP, a framework leveraging the gradient of the contrastive learning loss into the diffusion process to generate additional data with pseudo labels and desired labels. After delving into the desired properties of synthetic data contributing to the downstream classification task, they propose the optimal condition that the representation of different classes in data need to be more distinguishable in the synthetic distribution \cite{ouyang2023improving}. Via adopting the contrastive loss \cite{ouyang2023improving}. Contrastive-DP can explicitly control the distance between different classes of representational abilities to efficiently achieving adversarial robustness in classification tasks. In a comparison of the clean and adversarial accuracies of Contrastive-DP with conventional AI-based methods RoCL, AdvCL, and DeACL \cite{ouyang2023improving} on CIFAR-10 dataset, Contrastive-DP's accuracy surpasses the best of these methods by approximately 9\%. Specifically, while Contrastive-DP achieves an accuracy advantage of 59.99\%, the accuracy for RoCL, AdvCL, and DeACL are recorded at 47.88\%, 49.77\%, and 50.39\% respectively \cite{ouyang2023improving}. In the content of vehicular networks, attacks against neural network detectors are often so difficult to perceive that attack data collected by sensors is often sparse. These significant improvements of Contrastive-DP demonstrate the strong potential to improve the robustness neural network detectors for there sparse data attacks. 
    

\end{itemize}


\subsection{Attack Detection}

Adversarial Learning algorithms address the drawbacks of conventional AI-based detection systems, i.e., when facing new attacks, lacking of attack data and decreasing in the accuracy rate. within networks, there are several applications to detect attacks via GAI models:

%As we discuss in section \ref{Lim}, the AI-based detection systems have a significant drawback which is the lack of attack data leading a decrease in the accuracy rate of new attacks detection. Generative models, with the ability to model high-dimensional data distributions, alleviates the problem of insufficient abnormal samples to a certain extent. There are several applications to detect attack via GAI models:

\begin{itemize}
    \item \textbf{Intrusion Detection:} 
    Controller Area Network (CAN) is an essential part of vehicular networks providing communication between vehicles and Electronic Control Units (ECU)\cite{seo2018gids}. Due to the lack of security features, CAN is vulnerable against attacks needing to employ Intrusion Detection Systems (IDS) \cite{seo2018gids}. The primary drawback of the existing IDS methods deployed in CAN is their need for continuous updates especially when the in-vehicle environment changes, highlighting a challenge in maintaining consistent vehicular security. To address these problems, the authors in \cite{seo2018gids} propose Generative Adversarial Nets based Intrusion Detection System (GIDS) focusing on three aspects: effectiveness, expandability, and security. Since ECU in a vehicle generates about 2,000 CAN data per second \cite{seo2018gids}, using all the bits of the CAN data directly could take a long time and is not suitable for real-time detection. Inspired by powerful effects of GAI-aided detection for anomalous images, GIDS encodes CAN data with onehot-vector converted to image to keep effective. GAN in GIDS is used to generate fake images that are similar to real ones improving performances of the discriminator. Different from conventional GAN, GIDS consists of two discriminative models trained for known attack and unknown attack respectively to ensure expandability. To demonstrate the superiority, the authors test GIDS on a real vehicle (Hyundai’s YF Sonata) and four types of attacks (DoS, FUZZY, RPM, and GEAR) where Dos attack can inject high priority of CAN messages, Fuzzy attack can inject messages of spoofed random CAN ID and DATA values\cite{seo2018gids}. As results of the experiment, against all four attacks, the GIDS showed the average accuracy of 100\% for the first discriminator and the average accuracy of 98\% for the second discriminator\cite{seo2018gids}. These four types of attacks prevalent in vehicular networks pose significant threats to the communication infrastructure causing interruptions, degrade network performance, and, more critically, compromise the safety and security of vehicular operations. The high accuracy of GIDS experimental results highlights the power of leveraging GAI directly as a method for intrusion detection in vehicular networks.
    

    
    \item \textbf{Anomaly Detection:} The Cyber-Physical System (CPS) integrates computational elements with physical processes \cite{yan2022tfdpm}. As an essential part of vehicular networks, CPS enables real-time monitoring, decision-making, and control over vehicles, enhancing traffic management, safety, and vehicle-to-vehicle communication. Existing AI-based detection methods for CPSs usually adopt tractable distributions to approximate data distribution, which are not suitable for complex systems. To tackle this issue, the authors in \cite{yan2022tfdpm} propose TFDPM, a general framework for attack detection tasks in CPSs based on DMs and Graph neural networks. TFDPM consists of two components: pattern extraction module and conditional diffusion probabilistic module. In the first module, graph attention networks are utilized to explicitly model the correlation of data in different channels. In the second module, conditional DMs are employed to extract features at each time step performing prediction. In order to meet the requirements of online real-time detection, a conditional noise scheduling network is proposed to accelerate the prediction process of TFDPM. To assess the efficacy, they utilize three real-world CPS datasets: PUMP, SWAT, and WADI \cite{yan2022tfdpm}. Comparing with state-of-the-art attack detection methods, the best F1-scores on WADI and PUMP datasets based on TFDPM are about 4\% and 2\% higher than the best results of existing baselines respectively. For the SWAT dataset, TFDPM's performance is on par with the best of existing benchmarks \cite{yan2022tfdpm}. The CPS, as an important part of vehicular network communication, has multiple ECUs and sensors, making it more vulnerable to attack. These experiments demonstrate the efficacy and potential of TFDPM as a reliable method in the domain of attack detection in CPSs to secure the entire vehicle networks.
    
    \item \textbf{DDoS Attacks Detection:} Distributed Denial of Service (DDoS), as a distributed attack, causes significant damage to critical online services within vehicular networks. Recently, attackers have managed to keep their attacks below the threshold of threshold-based detection systems and modify their attacks to evade signature-based detection. Inspired by adversarial learning, the authors in \cite{abdelaty2021gadot} propose GADoT, a GAN-based adversarial training for robust DDoS attack detection. Within this framework, they exploit a GAN to generate fake-benign samples in order to perturb DDoS samples as adversarial examples. Then they use LUCID \cite{abdelaty2021gadot}, a lightweight and efficient DDoS detection system, as the target model training on the dataset augmented with perturbed samples. To demonstrate the enhanced ability of the GADoT, they consider two types of DDoS attacks: TCP SYN flood and HTTP GET flood \cite{abdelaty2021gadot} aiming at exhausting the victim’s resources by sending large amounts of requests to the victim server and making its services unavailable to the users. In experiments, after using GADoT for training, the detection accuracy in the case of delay perturbation experiences more than 43\% improvement in the F1 score, reaching 98.71\%. The same improvement is also apparent in the FNR that drops to 1.8\%, indicating the increased resilience to adversarial perturbations when trained with GADoT \cite{abdelaty2021gadot}. Compared to DoS attacks, DDoS attacks are more difficult to defend against because of their distributed nature, which makes them more threatening especially in vehicle networks with frequent communications. These improvements underscore an effective detection method that the model can adeptly and accurately detect DDoS attacks within networks with GAI‘s assistance.

    
    % \item \textbf{Generative AI Classifier:} Generative AI classifier means transforming a generative model into a classifier. Recently, the authors in \cite{li2023your} show a new perspective of conditional diffusion models viewing it as a Zero-Shot Classifier. Instead of generating a specific label images, they compute class-conditional likelihoods. Then they use predicted class probabilities of a input image to classify it. As a state-of-the-art method, their diffusion-based method shows stronger multi-modal compositional reasoning ability than discriminative AI approaches. In the content of classifying out-of-distribution data which can be seem as unknown attacks in vehicular networks, this diffusion classifier achieves much higher OOD accuracy on ImageNet-A than its ImageNet accuracy and achieves an effective robustness of 15-25\% compared 1-5\% in Resnet and 10-20\% in ViT.
\end{itemize}

\new{
\subsection{Identity Recognition}


Identity recognition in vehicular networks is a critical aspect of vehicular communication systems. It refers to the process of recognizing and verifying the identity of vehicles in a network to ensure secure and trusted communication. 

\begin{itemize}
    \item \textbf{Face Recognition:} Biometrics-based identification and verification techniques are considered as essential parts in security systems. For vehicle security and vehicular networks, face recognition is considered a good choice biometric technique since it based on human face feature information and can work under different conditions. Instead of using keys or smart cards, a vehicle could use face recognition through the interfaced of loT technology to authenticate the driver and grant access \cite{elngar2020vehicle}. Recently, several face recognition methods based on traditional AI have been introduced, aiming to enhance security within vehicular network \cite{elngar2020vehicle,lu2019intelligent,derman2018continuous,wang2019design}. Usually, these methods need to be trained on the public large-scale face recognition training databases \cite{cao2018vggface2, guo2016ms}. However, these datasets contain millions of images sourced from the internet without acquiring explicit user consent, which brings to the serious legal and ethical concerns regarding the utilization of these databases for facial recognition development. Under the terms of the General Data Protection Regulation (GDPR) \cite{deac2018regulation}, as well as other data protection regulations, there are stricter requirements imposed on the collection, distribution, and usage of face databases. Adhering to these regulations can be extremely challenging, and in some cases, nearly impossible, when maintaining these extensive databases \cite{boutros2023idiff}. 

    \textif{GAN:} 
    
    \textit{DMs:} Traditional generation methods often fail to ensure that synthetic images of synthetic identities have clear identity separability, with a desirable relatively large intra-class diversity. This leads to potential overlaps and ambiguities among different synthetic images, which complicates the process of clearly distinguishing them. To handle this issue, the authors in \cite{boutros2023idiff} propose IDiff-Face, a framework based on conditional latent diffusion models for synthetic identity generation. The first stage of IDiff-Face is to train an Autoencoder (AE) or use a pre-trained AE to project the training images into a latent space as the identity condition and then leverage the latent space for the second stage: DM training. Instead of directly inputting this representation into the DM, a Cross-Attention mechanism \cite{rombach2022high} is employed, ensuring the DM incorporates with the identity features throughout its training. To maintain the realism of synthetic data and prevent overfitting, Contextual Partial Droput (CPD) is introduced, which drops out components with a certain probability of the identity context \cite{boutros2023idiff}. Compared with the recent state-of-the-art synthetic datasets in terms of identity-separability and intra-class variation, IDiff-Face offers a more realistic trade-off between identity discrimination and intra-class variation. By utilizing IDiff-Face's synthetic data (500K images) for face recognition training, synthetic-based face recognition achieves an average accuracy of 88.20\%, significantly outperforming all state-of-the-art synthetic-based face recognition where the best average accuracy is 83.45\%. Moreover, IDiff-Face closes the gap to state-of-the-art face recognition trained on authentic data, where the average accuracy on CASIA-WebFace \cite{yi2014learning} (500K images) and MS1MV2 \cite{guo2016ms, deng2019arcface} (5.8M images) were 94.92\% and 97.18\%, respectively. Finally, compared with human-level performance in face verification where the reported accuracy on Labeled Faces in the Wild (LFW) \cite{huang2008labeled} is 97.5\%, IDiff-Face achieves 98.00\% \cite{boutros2023idiff}. With the rise of privacy policies, IDiff-Face provides a framework that generate datasets with distinct identity separability. These generated datasets enhance face recognition accuracy while addressing privacy concerns and simultaneously ensuring user identity recognition within vehicular networks, satisfying the security requirements.
 
\end{itemize}

\subsection{Privacy}

\begin{itemize}
    \item \textbf{Face Anonymization:} 
    Cameras, as an important sensor within vehicular networks, has become increasingly prevalent, capturing not only traffic patterns but also pedestrians and surrounding structures, especially of pedestrians' facial information, which poses significant privacy concerns in real-world scenarios. Face Anonymization aims to prevent the face identification algorithm from recognizing the real identity by changing the face image and doesn't affect recognition algorithms of non-portraits. Traditional privacy-protecting models blur face images through machine learning methods, but advanced deep learning can quickly identify the protected faces. As for deep learning methods, human faces may be deformed or blurred in feature level, making them difficult to maintain the naturalness of the human face, affecting seriously other recognition algorithms. Therefore, there's a need for the development of more advanced models that incorporate pixel-level and feature level naturalness preservation techniques.

    \textit{GAN:} Recently with the power of generative AI, several face deidentification models based on GAN have been proposed, such as CycleGAN \cite{zhu2017unpaired}. However, most of GAN-based models only makes the deidentification model protect identities at the pixel level, causing the protected images to be more easily recognized by deep learning face identification approaches. To address these issues, the authors in \cite{yang2023adversarial} propose a framework Adversarial Secret-identity Generation Model (ASGM) for face deidentification against black-box face recognition systems at both pixel-level and feature level. ASGM consists of two primary modules: an identity encryption GAN (IEGAN) and a potential face selection (PFS) approach. IEGAN is a face generator employing employs a CycleGAN method modified by residual blocks and self-attention layers.
    Via the adversarial and feature-protected loss functions, IEGAN can ensure the generated faces are not distorted from the human perspective. PFS aims to find the target set with the largest difference in feature level between real faces and target images, which can promote the model training at the sample level. To demonstrate the efficacy of ASGM, four state-of-the-art face identification algorithms were employed serving as Black Box Attacks: ArcFace \cite{deng2019arcface}, FaceNet \cite{schroff2015facenet}, CosNet \cite{zhang2020cross}, and SphereNet \cite{liu2017sphereface}. The protection capability of ASGM was assessed on the 'in the wild' dataset, specifically the Labeled Faces in the Wild (LFW) \cite{huang2008labeled}. ASGM outperforms other existing baseline network by a large margin in all face models \cite{yang2023adversarial}. Particularly, achieving 98.1\% R1-T, 99.2\% R5-T, 98.5\% R1-U, and 97.1\% R5-U against ArcFace, separately \cite{yang2023adversarial}. To facilitate ASGM in vehicular networks, the authors compress ASGM via a GAN compression method \cite{li2020gan}. The parameters of ASGM can be compressed by more than five times, causing only a minor loss in the face anonymization capability. With the guarantee of compressed model size and experimental effectiveness, ASGM emerges as a promising solution, underscore the profound potential of GAI in safeguarding face privacy within vehicular networks.

    \item \textbf{Location Anonymization:} Besides leaking facial information from pedestrians, several “over-needed information” captured by cameras within vehicular networks, such as street view background, license plate and model of surrounding vehicles, and others, can also become a breakthrough for attackers to steal privacy. Additionally, if the attacker manages to access a sequence of the victim's images that are time-correlated, it becomes feasible for them to deduce the victim’s potential route and estimate their driving speed \cite{xiong2019privacy}. It is crucial to preventing “over-needed information” of camera data from being attacked by location inference.

    \textit{GAN:} Although some existing methods aim to protect privacy of face information by Face Anonymization \cite{yang2023adversarial}, these methods only focus on keeping the context structure of small objects. Since the street view images have more complex context structures containing a variety of objects, the aforementioned methods are not suitable for protecting vehicular camera data. To address this issue, the authors in \cite{xiong2019privacy} propose a GAN-based framework: Auto-Driving GAN (ADGAN). ADGAN utilizes image-to-image translation to eliminate private objects in images while maintaining the utility of valuable objects, which strikes a trade-off between ensuring privacy and retaining utility. ADGAN consists of a generator built based on U-Net \cite{ronneberger2015u} and two discriminators to judge whether their inputs are the real images or the synthesized images. Instead of one discriminator only reads a certain part, combining two discriminators can enhance the ability to distinguish image, which provides privacy protection guarantee. To evaluate the performance of ADGAN, experiments in \cite{xiong2019privacy} adopte two different vehicular camera datasets: Cityscapes Dataset \cite{cordts2016cityscapes}, Google Street View \cite{zamir2014image}. Compare with the baseline pix2pix \cite{isola2017image} not considering privacy protection, the pixel accuracy of ADGAN for non-sensitive objects on Cityscapes Dataset and Google Street View is only reduced by 3\%, achieving 81.91\% and 78.97\% respectivel, where the best of other methods is only nearly 60\%. Although other methods can preserve more private information than ADGAN does on sensitive objects, they nearly lose all useful information and have worse recognition utility since the accuracy for non-sensitive objects is low. In the context of vehicular networks, especially for auto-driving, ensuring recognition accuracy is paramount. Therefore, ADGAN provides a more effective trade-off between privacy and utility compared with the state-of-the-art methods.

 
\end{itemize}

}

\subsection{Safety}




\begin{table*}
    \caption{Vehicular Network}
    \centering
    \begin{tabular}{c|c|c}
        \hline
        Application &  Technology & Reference\\\hline
        Adversarial Purification & GAN  &  \cite{samangouei2018defense} \\\hline
        ~ & DMs &  \cite{yoon2021adversarial,wu2022guided, wang2022guided,nie2022diffusion}\\\hline
        Adversarial Examples &  GAN   & \cite{lee2017generative} \\\hline
        ~ & DMs & \cite{ouyang2023improving, altstidl2023raising, gowal2021improving}\\\hline
        Intrusion Detection & GAN &\cite{seo2018gids} \\\hline
        ~ & DMs & \cite{yan2022tfdpm}\\\hline
        Generative AI classifier & DMs &  \cite{li2023your} \\\hline
        From survey & GAN & \cite{shu2020collaborative,ashraf2020novel} \\\hline
        Identity Recognition & DMs & \cite{boutros2023idiff} \\\hline
        Face Anonymization & GAN & \cite{yang2023adversarial} \\\hline
        %\multicolumn{2}{c}{name}\\
    \end{tabular}
\end{table*}

==> Network.tex <==
\section{Network Layer}

\begin{itemize}
    \item \textbf{Intrusion Detection}:
    \item \textbf{Privacy}:
\end{itemize}


\subsection{Problems}

\subsection{Security}


\subsubsection{Availability}

\begin{itemize}
    \item Denial-of-Service (DoS) Attack: A DoS attack is one of the most common attacks on vehicular networks. An attacker tries to chunk the main communication between vehicles and hence interrupt services. Therefore, the services are unavailable to the users in the network \cite{hasrouny2017vanet}. Distributed Denial of Service (DDoS) is a special type of DoS attacks, which can take place from multiple locations, making it more difficult to detect an attack \cite{zeadally2012vehicular}.
    \item FUZZY Attack: A FUZZY attack is a common type of injection attacks launched on Controller Area Network (CAN) bus. An attacker injects random or malformed messages at a high frequency to overwhelm the Electronic Control Units (ECUs) in vehicles. The attack causes vehicles to display unexpected states or fail \cite{swessi2022comparative}.
    \item Bus-off Attack: A bus-off attack is a type of DoS attacks exploit the error-handling scheme of in-vehicle networks. An attacker periodically injects attack messages to the in-vehicle network, deceives uncompromised ECUs to disconnect or shut down them \cite{cho2016error}.
    \item Malfunction Attack: A malfunction attack, also called the fault attack, is a type of cyber attack where the attacker deliberately induces faults in a computing system to compromise its security. The induced faults can disrupt the normal operation of the system, causing it to reveal sensitive information or behave in unintended ways \cite{han2021ppm}. 

\end{itemize}

\subsubsection{Confidentiality}

\begin{itemize}
    \item Masquerade Attack: In a masquerade attack, an attacker disguises themselves as a legitimate user or device to bypass security measures and gain unauthorized access. This attack often involves the appropriation or impersonation of legitimate user credentials, such as usernames and passwords \cite{azees2016comprehensive}.
    \item SOME Attack: A SOME attack is a more advanced type of masquerade attacks. The attack can imitate normal message frequencies from a regular ECU and keep the same ID sequence on the CAN bus. It can also send harmful information that appears the same as normal messages since the attack comes from the same ECU \cite{zhao2022gvids}.
    \item User to Root (U2R) Attack: An U2R attack is a a type of cyber-attack where an attacker begins with access to a normal user account on the system and exploits vulnerabilities to gain root access, which allows the attacker to perform any actions, including those that can harm the system or compromise sensitive data \cite{alharbi2018denial}. 
    \item Remote to Local (R2L) Attack: A R2L attack is conceptually similar to the U2R attack, but the methods used are different. In an R2L attack, an attacker from a remote location exploits vulnerabilities in a network or system to gain local access. R2L attacks can lead to unauthorized data access, data theft, or further exploitation of the network's internal resources \cite{alharbi2018denial}.
    \item Probing Attack: A probing attack present a significant risk to collaborative intrusion detection systems. An attacker identify open ports, running services, and system weaknesses, which sets the stage for more targeted and damaging attacks through methods like port scanning and packet analysis \cite{alharbi2018denial}.
    
\end{itemize}


\subsubsection{Integrity}

\begin{itemize}
    \item RPM or GEAR Spoofing Attack: In vehicular networks, the car's engine speed (RPM) and gear settings play a crucial role. An attacker aims to inject messages related to RPM/GEAR information to influence the vehicle operation. This can cause problems with how the car runs and might even lead to unsafe driving conditions \cite{seo2018gids}.
    \item Replay Attack: A replay attack is also known as a playback attack, where  a valid data is maliciously or fraudulently retransmitted or delayed. An attacker  intercepts and stores data, such as authentication tokens, and then retransmits it to produce an unauthorised effect \cite{azees2016comprehensive}.
\end{itemize}




\subsection{Traditional AI methods}



\subsection{Generative AI methods}


\begin{table*}[htp] \footnotesize
  \centering
  \caption{Your table caption here.}
  \label{tab:my_label}
    \begin{tabular}{m{0.05\textwidth}<{\centering}||m{0.11\textwidth}<{\centering}|m{0.08\textwidth}<{\centering}|m{0.32\textwidth}<{\centering}|m{0.32\textwidth}<{\centering}}
      \hline
      \textbf{Ref} & \textbf{Attack}  & \textbf{Algorithm} & \textbf{Pros} & \textbf{Cons} \\
      \hline
      \cite{seo2018gids}  & DoS, FUZZY, RPM, GEAR & GIDS  & \begin{itemize}[leftmargin=*]
          \item[-] Encode CAN data with onehot-vector
          \item[-] Two discriminative models trained for known attack and unknown attack
      \end{itemize}
      & \begin{itemize}[leftmargin=*]
      \item[-] Consist of the complicated structure and need relatively long training time
      \item[-] Cannot distinguish normal traffic from anomalous traffic
      \end{itemize}\\
      \hline
      \cite{yang2021intrusion}  & DoS, FUZZY, RPM, GEAR & GAN-based IDSs  & 
      \begin{itemize}[leftmargin=*]
      \item[-] A discriminator that can distinguish five categories
      \item[-] Relatively simple network structure
      \end{itemize}
      &
      \begin{itemize}[leftmargin=*]
      \item[-] The CAN message block is constructed roughly
      \item[-] Focus on certain types of attacks
      \end{itemize}\\
      \hline
        \cite{xie2021threat}  & DoS, Masquerade & GAN-based IDSs  & 
        \begin{itemize}[leftmargin=*]
      \item[-] Introduce the CAN communication matrix defined by the OEM
      \item[-] An enhanced GAN discriminator trained by the CAN communication matrix
      \end{itemize}
      &
      \begin{itemize}[leftmargin=*]
      \item[-] Unsuitable for large-scale deployment
      \item[-] Cannot handle ever-changing attacks
      \end{itemize}\\
      \hline
      \cite{chen2021intrusion} & DoS, FUZZY, RPM, GEAR & ACGIDS  & 
      \begin{itemize}[leftmargin=*]
      \item[-] Replace RFC in GAN by additional double classifiers
      \item[-] Propose an offline detection process 
      \end{itemize}
      &
      \begin{itemize}[leftmargin=*]
      \item[-] High-dimensional space solution is expensive in time
      \item[-] Require relatively long training time 
      \end{itemize}\\
      \hline
      \cite{zhao2022can}   & DoS, FUZZY, RPM, GEAR & ACGAN-AC-RFCTh  & 
      \begin{itemize}[leftmargin=*]
      \item[-] Combine with OOD detection methods
      \item[-] Employ a multi-class Auxiliary Classifier
      \end{itemize}
      &
      \begin{itemize}[leftmargin=*]
      \item[-] Require secure network architectures for advanced attacks
      \item[-] Unsuitable for large-scale deployment
      \end{itemize}\\
      \hline
        \cite{hoang2022detecting}   & DoS, FUZZY, RPM, GEAR & CAAE-based IDS & 
        \begin{itemize}[leftmargin=*]
      \item[-] Lightweight and suitable for real-time deployment
      \item[-] Require only a small amount of labeled data 
      \end{itemize}
      &
      \begin{itemize}[leftmargin=*]
      \item[-] Require a different data preprocessing depending on the structure of the new attacks dataset 
      \end{itemize}\\
      \hline
      \cite{wang2023transfer}  & DoS, FUZZY, RPM, GEAR & TLSIDS  & 
       \begin{itemize}[leftmargin=*]
      \item[-] Form a cascade detection system to prevent from missing unknown attacks
      \item[-] Consist of the self-learning function to automatically update the model
      \end{itemize}
      &
      \begin{itemize}[leftmargin=*]
      \item[-] The low-value ID of DoS attacks may not really exist in real-world situations
      \end{itemize}\\
      \hline
      \cite{zhao2022gvids}  & Spoofing, Bus-off,  Masquerade, SOME & GVIDS  & 
      \begin{itemize}[leftmargin=*]
      \item[-] The ability to detect novel attacks like SOME attacks
      \item[-] Good detection and high real-time performance in real-world situations
      \end{itemize}
      &
      \begin{itemize}[leftmargin=*]
      \item[-] Lack the verification of the robustness in more complex environments
      \end{itemize}\\
      \hline
       \cite{kavousi2020evolutionary}  & Fake message traffic & MFA-GAN  &
       \begin{itemize}[leftmargin=*]
      \item[-] Combine the GAN framework with FA
      \item[-] Three-stage modification solution for FA to avoid premature convergence and increase the population diversity
      \end{itemize}
      &
      \begin{itemize}[leftmargin=*]
      \item[-] Cannot employ online learning
      \item[-] Rely on a suitable fitness function
      \end{itemize}\\
      \hline
      \cite{han2021ppm}  & DoS, FUZZY, Malfunction, Replay & PPM-InVIDS  & 
      \begin{itemize}[leftmargin=*]
      \item[-] Transform CAN shallow features into complex-valued features to protect privacy 
      \end{itemize}
      &
      \begin{itemize}[leftmargin=*]
      \item[-] Rely on the performance of pre-trained GAN models
      \end{itemize}\\
      \hline
    \cite{shu2020collaborative }  & DOS, U2R, R2L, Probing & CIDS & 
    \begin{itemize}[leftmargin=*]
      \item[-] Jointly train an effective detection model for the entire network
      \item[-] Prove the correctness of CIDS in both IID and non-IID situations
      \end{itemize}
      &
      \begin{itemize}[leftmargin=*]
      \item[-] The hyperparameter impacts the balance between effectiveness and communication cost
      \end{itemize}\\
    \hline
    \cite{li2022gan}  &  anomaly message & CAN  & Detection & GAN \\
    \hline
    \end{tabular}
\end{table*}


\textit{1) Using GAI to handle intrusion detection in the Controller Area Network (CAN):}

As an essential part of vehicular networks, Controller Area Network (CAN) is a standard of the bus system for in-vehicle network providing communication between vehicles and Electronic Control Units (ECU) \cite{lokman2019intrusion}. Due to the lack of security features, CAN is vulnerable against attacks needing to employ Intrusion Detection Systems (IDS). Although existing traditional AI methods are efficient in IDS, they have certain limitations. Especially when in-vehicle environments changing, they need to update to be familiar with new attacks. Furthermore, if the details of IDS are leaked to attackers, the attackers could potentially manipulate the system and evade detection. 

To address these problems, the authors in \cite{seo2018gids} propose GAN based Intrusion Detection System (GIDS) (shown as Fig \ref{fig:GIDS}), which can learn to detect unknown attacks using only normal data. Since ECU in a vehicle generates about 2,000 CAN data per second \cite{seo2018gids}, using all the bits of the CAN data directly could take a long time and is not suitable for real-time detection. Inspired by powerful effects of GAI-aided detection for anomalous images, GIDS encodes CAN data with onehot-vector converted to image to keep effective. GAN in GIDS is used to generate fake images that are similar to real ones improving performances of the discriminator. Different from conventional GAN, GIDS consists of two discriminative models trained for known attack and unknown attack respectively to ensure expandability. To demonstrate the superiority, the authors test GIDS on a real vehicle: Hyundai’s YF Sonata, and four types of attacks: DoS, FUZZY, RPM, and GEAR, where Dos attack can inject high priority of CAN messages; Fuzzy attack can inject messages of spoofed random CAN ID and DATA values; RPM and GEAR attack inject messages of certain CAN ID related to RPM/GEAR information \cite{seo2018gids}. As results of the experiment, against all four attacks, the GIDS showed the average accuracy nearly of 100\% for the first discriminator focusing on known attacks and the average accuracy of 98\% for the second discriminator concentrating on unknown attacks \cite{seo2018gids}. 

\begin{figure}[htp]
    \centering
    \includegraphics[width= 0.95\linewidth]{figs/GID.pdf}
    \caption{The overall architecture of the GIDS \cite{seo2018gids}. \textit{Part A} demonstrates the training procedure for known attacks, where the first discriminator is trained by abnormal data and normal data. In \textit{Part B}, the generator and the second discriminator are trained simultaneously by the adversarial process to improve the detection ability for unknown attacks. \textit{Part C} illustrates the detection procedure, where the input CAN images are firstly sent to the first discriminator and then those passing the first judgment are sent to the second discriminator for further detection according to the given threshold.}
    \label{fig:GIDS}
\end{figure}



Even though GIDS demonstrates strong detection ability both on known and unknown attacks, it relies on two discriminative models, which is too complicated to decrease training and detection time. Moreover, DNN still contributes the most part for accuracy rather than GAN, according to their experiments. To simplify models and improve detection ability, the authors in \cite{yang2021intrusion} proposed GAN-based IDSs for the in-vehicle network. Compared with GIDS \cite{seo2018gids}, this model architecture consists of one improved GAN, including a discriminator and a generator, which extends the capability to perform five-class classification indicating specific attack types: normal data, DoS attacks, FUZZY attacks, RPM attacks, and GEAR attacks, instead of the binary classification as normal or attack states. To save training and detection time, the proposed model requires fewer layers where the discriminator includes two convolution layers and two linear layers with a new loss function, and a smaller format size of input data. To demonstrate superiority, this model compared with GIDS and are better by 1–3\% on metrics of detection, precision, and accuracy  \cite{yang2021intrusion}. Moreover, as for detecting a single CAN images, the time is $0.12 \pm 0.03$ ms.

In the prepossessing phase of GIDS \cite{seo2018gids} and the proposed model in \cite{yang2021intrusion}, one CAN message block is constructed by specific number of consecutive CAN message jobs which is rough and cannot accurately reflect the actual CAN message block. In addition, they only focus on certain types of attacks and fail to detect the data tampering threat which can also achieve serious destructiveness. To solve these limitations, the author in \cite{xie2021threat} introduce the CAN communication matrix defined by the automotive Original Equipment Manufacturer (OEM) for a vehicle model into GAN model-based IDSs. Leveraging the message sending type in the CAN communication matrix, a CAN message block is from the same CAN message and all CAN message jobs have the same message identifier. This approach guarantees that the constructed CAN message blocks in the training dataset accurately represent the actual CAN message blocks that would be generated during the detection phase. Then, they train an enhanced GAN discriminator via the CAN communication matrix, which can discriminate whether each message has suffered from the data tampering threat and increase the detection accuracy. In experiments, the proposed method and the method in \cite{yang2021intrusion} both have high performance against DoS attacks. When against the data tampering threat, even though they can perform effective, the method in \cite{yang2021intrusion} shows a high recall as 99.9\% and the proposed method is extremely low to 1\% \cite{xie2021threat}. 

Although the above methods combine DNN and GAN to improve the detection accuracy of unknown attacks, the multi-stage model's complexity makes it unsuitable for large-scale deployment. Additionally, it requires a small amount of attack data to be incorporated during the training stage, which complicates adaptability to handle ever-changing attacks. Inspired by the method in \cite{barletta2020intrusion} whose data dimension is so larger that requires large memory resources, the authors in \cite{chen2021intrusion} propose an intrusion detection method based on auxiliary classification against network (ACGIDS) to solve the previous problems. Within this framework, the generator is designed to adapt to distributions that diverge from normal data, thereby covering patterns associated with unknown attacks. Concurrently,  to circumvent issues caused by the discriminator degradation \cite{zenati2018adversarially,kong2021opengan}, the traditional GAN's real-fake classifier (RFC) is replaced by additional double classifiers. These classifiers serve as the foundational elements for anomaly detection, ensuring robustness against the discriminator's performance variability. They also design an offline detection process that is both dependable and easy to deploy, which utilizes two classifiers to sort known and unknown data types without requiring a preset threshold. According to the experiments on the CAN dataset \cite{song2020vehicle, seo2018gids}, considering the unknown DoS dataset, the F1-Score of ACGIDS is as high as 99.45\%, where GIDS is 93.32\%. In the supervised scenario on the known attack dataset, the F1-Score of ACGIDS and GIDS are 99.63\% and 98.88\%, respectively \cite{chen2021intrusion}. The superior performance demonstrates the effectiveness of introducing adversarial training and the capacity to accommodate unknown anomaly patterns. Moreover, in terms of inference speed, ACGIDS needs $1.27$ ms where GIDS needs $4.39$ ms. In terms of parameter storage size, ACGIDS and GIDS need 0.46MB and 0.49MB, respectively \cite{chen2021intrusion}. 

In actual attacks, attackers usually mix known attacks and novel zero-day attacks. Therefore, it is important for IDs to assign fine-grained labels and detect any unknown attacks. When considering the problem formulation of multi-class classification: Normal, Known Attacks, and Unknown Attacks, the authors in \cite{zhao2022can} propose four methods, similarly to \cite{chen2021intrusion} , where the best-performing method ACGAN-AC-RFCTh is the one based on Auxiliary Classifier Generative Adversarial Network (ACGAN) \cite{odena2017conditional} in combination with Out-of-Distribution (OOD) detection \cite{hendrycks2016baseline}. The ACGAN-AC-RFCTh is a cascaded two-stage classification architecture. In the first stage, a multi-class Auxiliary Classifier (AC) is tasked with classifying samples as either normal or known attacks. In the second stage, OOD detection serves as the initial filter to separate unknown attacks from normal messages, where OOD samples refer to data points that deviate from the distribution represented in the training dataset. Subsequently, the Real-Fake Classifier (RFC) within the GAN framework is utilized for the final classification of the unknown attack category. Evaluated on the public car-hacking dataset \cite{carhacking2018}, it achieves F1-score of 99.28\%, 99.15\%, 99.53\%, and 99.80\% for DoS, FUZZY, GEAR, and RPM attacks, respectively \cite{zhao2022can}.

The main challenge of IDS is a requirement of extensive labeled data for training, which is often costly and time-consuming to gather. By leveraging semi-supervised learning and generative AI, the model can effectively learn from a larger pool of unlabeled data while still benefiting from the precision that labeled data provides. In order to meet the real-time requirement for the in-vehicle IDS and simplify the complicated data prepossessing, the authors in \cite{hoang2022detecting} propose convolutional adversarial autoencoder (CAAE) based IDS by combining convolutional autoencoder and generative adversarial networks (GAN). The training process for CAAE includes a reconstruction phase focusing on the autoencoder part and a regularization phase where both the generator and discriminators are trained in an adversarial manner. The Wasserstein GAN (WGAN) loss with gradient penalty (GP) is used to stabilize the model and ensure convergence \cite{hoang2022detecting}. Their experiments on the car hacking dataset \cite{song2020vehicle} demonstrate that the proposed model can detect various types of message injection attacks, including DoS, FUZZY, and spoofing attacks, with a high F1 score of 99.84\% and a low error rate of 0.1\% \cite{hoang2022detecting}. The model is lightweight and suitable for real-time deployment, with a significant nearly 4 times reduction, in the number of model parameters and inference time is compared to other traditional AI models \cite{hoang2022detecting}.

\begin{figure}[htp]
    \centering
    \includegraphics[width= 0.95\linewidth]{figs/TBD.png}
    \caption{Pending. VAE+AE
    \textit{Part A} demonstrates the training procedure for known attacks, where the first discriminator is trained by abnormal data and normal data. In \textit{Part B}, the generator and the second discriminator are trained simultaneously by the adversarial process to improve the detection ability for unknown attacks. \textit{Part C} illustrates the detection procedure, where the input CAN images are firstly sent to the first discriminator and then those passing the first judgment are sent to the second discriminator for further detection according to the given threshold.}
    \label{fig:GIDS}
\end{figure}

While these methods can identify unknown attacks without updates, the detection capabilities of the IDS still need enhancement since the safety of drivers could be at risk even with a small number of undetected attacks. Transfer learning is a method where a model applies pre-learned knowledge to enhance intrusion detection, particularly useful when there is a shortage of labeled data available for training \cite{pan2009survey}. Even though many traditional AI methods are based on this, which has enhanced the detection capabilities for unknown attacks, the methods to acquire unknown attacks are missing. To handle these problems, the authors in \cite{wang2023transfer} propose a transfer learning-based self-learning IDS (TLSIDS) for CANs. In this framework, a GAN is utilized as an advanced detection module (ADM) for further detecting unknown attacks hidden in normal traffic detected by DenseNet in basic detection module (BDM). The GAN in ADM consists of a generator which is used to generate forged unknown attacks and a discriminator used as the unknown attack detection model. Then in unknown attacks classification module (UACM), the unknown attack samples stored by the ADM are classified and tagged to constructs new labeled training datasets for transfer learning. Finally, the self-learning module (SLM) trains transferred DenseNet. Evaluating TLSIDS on dataset provided by \cite{song2018network},  the results demonstrate that the TLSIDS could achieve a recall, precision, and F1-score of 99.97\%, 99.90\%, and 99.93\%, respectively, where GIDS's are 97.75\%, 98.2\%, and 97.97\% \cite{wang2023transfer}.

Even though the models mentioned previously can distinguish common attacks like DoS, FUZZY and spoofing attacks, some novel attacks, such as masquerade attacks \cite{miller2015remote,cho2016fingerprinting} and bus-off attacks \cite{cho2016error}, can easily bypass IDS models due to relatively few studies. Recently, the researchers in \cite{zhao2022gvids} discovered the same origin method execution (SOME) attack which is a highly camouflaged attack method in vehicular networks. The intrusion message of SOME attack has the same period, clock skew and voltage as the normal message making them difficult to differentiate from normal data using existing IDS models. To deal with SOME attacks, the researchers in \cite{zhao2022gvids} also proposed a reliable vehicle IDS based on GAN (GVIDS) \cite{zhao2022gvids}, which can detect not only SOME attack but also other existing attacks, including spoofing, bus-off and masquerade attacks. The GVIDS utilizes one-hot encoding with an adopted GAN known as GANomaly \cite{akcay2019ganomaly}. To evaluate the performance of the GVIDS on two real vehicles Luxgen U5 and Buick Regal, the area under curves values of spoofing, bus-off, masquerade, and SOME attacks in Luxgen are 0.9941, 0.9787, 0.9768, and 0.976 respectively, where the values are 0.9982, 0.9778, 0.9665, and 0.9662 in Buick \cite{zhao2022gvids}. Moreover, it has high real-time performance: each detection requires only 0.18 ms which can meet the demand of the detection of vehicular networks in real-time.


From the perspective of improving GAI model, most of the models discussed previously aim to minimize the model size and subsequently enhance the speed of training and prediction by employing a single generator and discriminator pair. However, the original GAN framework with a single generator has a significant drawback: it often exhibits unstable performance when dealing with highly nonlinear datasets, such as those involving unknown attacks, as noted in \cite{kavousi2020evolutionary}. This instability is a critical challenge, especially in scenarios where attackers employ a mix of known and unknown attack strategies. To address this issues, an evolutionary GAN based on firefly algorithm (FA) is proposed in \cite{kavousi2020evolutionary}. The FA is a meta-heuristic optimization algorithm inspired by the mating behavior of firefly insects found in tropical regions \cite{kavousi2014optimal}. With the help of the FA, a set of generators can be utilized to overcome the instability issues in the GAN instead of a single generator. Furthermore, to avoid premature convergence and increase the population diversity, a three-stage modification solution based on some powerful math operator for FA is proposed focusing on the convergence rate, the position of each firefly, and the dynamic randomization. Following modifications, the proposed model demonstrates so notable improvements that it not only achieved convergence faster than other evolutionary algorithms without modifications, indicating a high convergence rate, but also results in a better detection rate \cite{kavousi2020evolutionary}. Moreover, when detecting fake message traffics, the proposed model also achieves the highest hit rate, and correct reject rate by 96.84\% and 94.21\%, respectively, where the highest rate of the rest four SVM models \cite{avatefipour2019intelligent} is nearly 3\% lower \cite{kavousi2020evolutionary}.

\begin{figure}[htp]
    \centering
    \includegraphics[width= 0.95\linewidth]{figs/TBD.png}
    \caption{Pending. VAE+AE
    \textit{Part A} demonstrates the training procedure for known attacks, where the first discriminator is trained by abnormal data and normal data. In \textit{Part B}, the generator and the second discriminator are trained simultaneously by the adversarial process to improve the detection ability for unknown attacks. \textit{Part C} illustrates the detection procedure, where the input CAN images are firstly sent to the first discriminator and then those passing the first judgment are sent to the second discriminator for further detection according to the given threshold.}
    \label{fig:GIDS}
\end{figure}

(seems like data augmentation)
From the perspective of improving generated dataset, while the aforementioned models mainly aim to create additional data that's hard to differentiate for the discriminator, the generated data may not conform to the real message protocol specification and introduce some useless information. To generate messages conforming to the in-vehicle CAN protocol specification, the authors in \cite{li2022gan} proposed the field associated mutation generation adversarial network (FAMGAN) based on the Wasserstein generative adversarial network gradient penalty (WGAN-GP) \cite{arjovsky2017wasserstein}. The FAMGAN utilizes the bit transition rate within CAN messages to segment the data field whose effectiveness is verified by conditional random fields (CRFs) \cite{sutton2012introduction}. To further enhance the process, the FAMGAN applies the Apriori algorithm \cite{al2014improved} for association mining within the CAN message fields to extract their relationship, which can improve the similarity between the generated and tested messages. Therefore, the FAMGAN model takes advantage of protocol-based fuzz testing and machine learning-based fuzz testing \cite{fowler2018fuzz}. By sending the special test cases messages to the CAN bus of the vehicle, the RPM and vehicle speed on the instrument panel changed, where the RPM reached 7000 r/min, and the driving speed reached 156 km/h, while the car was not actually in a driving condition \cite{li2022gan}. The results of simulations show that the FAMGAN model can efficiently generate CAN messages that trigger vehicle anomalies in in-vehicle CAN networks. Consequently, FAMGAN plays a crucial role in bridging the gap between datasets collected from real vehicles and anomalous messages that fulfill the coverage requirements needed for effective intrusion detection algorithms. 

\todo{link data augmentation and IDS}

Deep Learning-based IDS achieve accurate detection by processing vast amounts of data, which often includes sensitive information. This practice raises significant privacy concerns for the deep learning models employed. Through leaked private data, attackers can not only design new attacks but also obtain sensitive information, which also reduces the reliability and accuracy of IDs. To protect the middle layer characteristics of IDS, the authors in \cite{han2021ppm} proposed the privacy protection model for in-vehicle IDS based complex valued neural network (PPM-InVIDS). The encoder module of the PPM-InVIDS consists of two sub encoders: an autoencoder and a WGAN-based encoder \cite{arjovsky2017wasserstein}, where the autoencoder decreases the complexity of high-dimensional data and the WGAN-based encoder converts the feature matrix into a complex-valued form and hides in random phases. As the model reaches convergence, the encoder loss is anticipated to follow a uniformly random distribution of the random phases. Therefore, when an adversary attempts to reconstruct the original input by randomly rotating the angle, it will generate an infinite number of features. Consequently, the abundance and variability of features effectively protect the input information, making it practically impossible for adversaries to deduce or infer the original input data from the multitude of generated features. Besides, it also demonstrates superior performance in the comparison experiment. The detection accuracy of PPM-InVIDS is 99.3\%, while GIDS \cite{seo2018gids} is 98.9\%. However, due to the more complex structure of PPM-InVIDS, the running time has also increased by 10\% compared to GIDS \cite{han2021ppm}.


\textit{2) Using GAI to handle intrusion detection in VANET:}

As a classical application of vehicular networks, the Vehicular Ad hoc Network (VANET) provides intelligent communication channels between vehicles and nearby roadside units (RSUs) \cite{manvi2017survey}. Due to the high complexity of topology, high mobility of vehicles, and diversity of communications, VANETs are also vulnerable to various cyber-attacks. However, most of existing traditional AI methods are built based on a part of the whole VANET, and limited to detect specific attacks under its local sub-network rather than the entire VANET.

To handle these problems, the authors in \cite{shu2020collaborative} proposed a collaborative intrusion detection system based on distributed SDN (CIDS), where SDN denotes Software defined networking a promising approach to provide a flexibility and programmability of network security control \cite{sahay2019application}. The CIDS is designed based on two GAN models: MD-GAN \cite{hardy2019md} and EGBAD \cite{zenati2018efficient} with multi-discriminators to train multiple distributed SDN controllers jointly. This approach addresses the biased flow problem seen in individual detection and reduces system computation and communication burdens compared to centralized detection. Additionally, the correctness of the CIDS under both IID (Independent Identically Distribution) and non-IID situations is proved theoretically in \cite{shu2020collaborative}. To evaluate the performance, both IDD and non-IID detection are considered on a intrusion dataset KDD99 \cite{KDD99_2010}. The results show that the accuracy of each distributed SDN is over 98\% on both situations \cite{shu2020collaborative}.

\todo{\textit{2) Using GAI to enhance privacy in network layer:}}


% (also data augmentation))

% \cite{rosenstatter2023towards}


% Deep generation models for continuous-valued sequences
% such as time series have been drawing a great amount of
% attention in a variety of applications. The closest to our work
% is the generation of in-vehicle signals for testing low-level
% vehicle control software. Parthasarathy et al. [14] applied
% the Variational Autoencoder-Generative Adversarial Network
% (VAE/GAN) architecture to learn an unlabelled dataset of
% recorded in-vehicle signals and use it for the generation of
% synthetic input stimulus. To capture characteristics that are
% interesting for the test and customise stimulus generation, they
% introduced a template and metric-based linear interpolation
% algorithm. Parthasarathy et al. [15] improve on the work
% above by introducing a simpler way of using templates to
% set explicit objectives for domain adaptation. Moreover, they
% utilise unsupervised disentanglement representation to enrich
% the generation of the test stimulus. In [16], Zec et al. train
% a recurrent GAN to generate a time series of automotive
% perception sensors for simulation-based verification. In [17]
% and [18], the authors have applied convolutional GANs for
% sequence generation. Both works use a mixture density network and Wasserstein-1, while the latter additionally performs k-means clustering to evaluate the effectiveness of the
% generated synthetic time series datasets. Another method is
% TimeGAN [19] that generates realistic time series data from a
% leaned embedding space which in turn is optimised with both
% supervised and adversarial objectives.


% \cite{parthasarathy2020controlled}

% These four types of attacks prevalent in vehicular networks pose significant threats to the communication infrastructure causing interruptions, degrade network performance, and, more critically, compromise the safety and security of vehicular operations.







==> Physical.tex <==
\section{Physical Layer}

\subsection{Problems}

Physical layer is the first layer of the Open Systems Interconnection (OSI) model, which is responsible for the management and maintenance of the physical data transmission medium \cite{kumar2014osi}. With an increasing number of wireless devices and the development of 5G or higher networks, information security has been a critical issue in wireless communication paying more attention to physical layer of security \cite{wu2018survey}. From the perspective of information theory, physical layer security technology primarily focuses on utilizing the natural propagation traits of wireless channels.

\begin{itemize}
    \item \textbf{Eavesdropping}: Eavesdropping in wireless communication represents a significant security concern. This type of attack involves intercepting and accessing confidential information transmitted over vehicular networks \cite{sheikh2019survey}. When an eavesdropping attack is implemented, the attackers can steal user identity and data location, which may be used to track the vehicles.
    \item \textbf{Jamming}: 
    \item \textbf{Authentication}:
    \item \textbf{Other Attacks}:

    
\end{itemize}

\subsection{Traditional AI methods}




\subsection{Generative AI methods}

% \cite{ding2024gan} A GAN-based security strategy for WSN networks based on honeypot algorithm
% (strategy)

% \pending{

% Owing to constrained resourceof sensor nodes, a significant level of
% redundancy, network data’s higher correlation,intrusion detection schemes for wireless sensor networks also
% have the drawbacks ofpoor identification rate, high computation overhead, and higher false alarm rate.

% Tooverwhelm
% the above problems, in this manuscript, Self-Attention-Based ProvisionalVariational Auto-Encoder
% Generative Adversarial Network (SAPVAGAN) optimized withHoney Badger Algorithms proposed for
% enhancing Cyber security in Wireless sensornetwork(ECS-WSN-SAPVAGAN–HBA).

% Based on the optimum features,
% the intruders in WSN data are categorizedinto normal and anomalous data (Black hole attack, Gray hole
% attack, Flooding attackand Scheduling attacks) with the help of SAPVAGAN.In general, SAPVAGANnotexpose
% any adaption of optimization modes for determining better parameters toassure accurate detection of WSN
% intrusion.

% Takeaways:
% The SAPVAGAN optimized with Honey Badger Algorithm (ECS-WSN-SAPVAGAN-HBA) effectively detects intrusions in WSNs.
% The use of GAN (Generative Adversarial Network) and Honey Badger Algorithm enhances the accuracy of intrusion detection.
% This method shows significant improvements over existing methods in terms of prediction accuracy and sensitivity.
% Practical Implications: The strategy can be applied in diverse WSN applications for more secure and reliable operations.
% Potential Impact: Could set a new standard for intrusion detection in WSNs, influencing future cybersecurity strategies.


% Unfortunately, gives a major challenge achieve this objectives in the
% unnatural resources ofWSNs together with storage,rectifying capacity
% and battery energy [5,6]. Such features givestraditional safety measures
% such cryptography not always enough like networks [7]. WSNsare very
% exposed the possibility of being attacked, due to their unlocked and
% shared natureand small materials of the detector nodes

% Existing methods for intrusion detection increase time consumption
% while also not offeringhigh accuracy and detection rates. Some conventional
% network intrusion detection techniquesare no longer useful
% since WSNs differ from typical computer networks in many ways,
% including terminal kinds, data transfer, network topology, and a number
% of other areas. IDSmust be highly accurate when identifying intruders,
% involving unknown attacks, itwellsituatedto make sure low overhead in
% WSN communication. These are the two keyrequirements when creating
% IDS for WSN. Hence, in this manuscriptSAPVAGANoptimizedwith
% Honey Badger Algorithm is proposed for intrusion detection scheme
% whichconform theproperties of WSN.

% "Owing to constrained resource of sensor nodes, intrusion detection schemes for wireless sensor networks also have the drawbacks of poor identification rate, high computation overhead, and higher false alarm rate"【98†source】.
% "The proposed ECS-WSN-SAPVAGAN–HBA method is performed in Python utilizing the WSN-DS dataset"【98†source】.
% "The performance of the proposed ECS-WSN-SAPVAGAN-HBA method provides higher prediction accuracy" compared with existing methods【106†source】.


% List: Specific limitations are not detailed in the quoted sections, but potential limitations could include the complexity of the method, computational resource requirements, and the need for specialized knowledge for implementation.
% Mitigations: Not discussed in the document.

% }









% \cite{lang2023radar} Radar-Based Noninvasive Person Authentication Using Micro-Doppler Signatures and Generative Adversarial Network

% \pending{

% This article presented a new strategy for noninvasive user
% authentication using human gait micro-Doppler signatures.

% authentication


% In this context, nonintrusive sensors are more desired in
% real-life applications. Radar, due to its inherent remote sensing
% properties, can capture gait at a distance without the
% subjects’ awareness. Besides, being propelled by its electromagnetic
% sensing modality, radar is applicable in situations
% with poor light conditions or occlusion (which are severedisturbances in the visual perception systems). Some recent
% advances in radar-based human analysis have been credited
% to the micro-Doppler signatures [12], [13], [14], [15], [16],
% [17]. By providing useful micro-movement information, the
% micro-Doppler signatures have been proven effective in characterizing
% human activities.

% }




==> Problem.tex <==
\section{Security and Privacy in Vehicular Network}\label{Pre}

In this section, we first introduce the principal security and privacy threats prevalent in vehicular networks. Then, we discuss several AI-based methods security solutions for vehicular networks especially about their limitations.

\subsection{Security and Privacy Threat}

Based on the type of attack, the security threats on vehicular networks can be categorized into the following four classes: 

\begin{itemize}
    \item \textbf{Hardware or Software (HW/SW)-Based Attack:} These attacks take place over the hardware components and software systems of vehicular networks, such as Timing Attack, GPS Spoofing, and Routing Attack etc.
    \item \textbf{Infrastructure-Based Attack:} These attacks target the foundational structures that support vehicle operations, aiming to compromise the integrity, and availability of vehicular services. Several attacks infecting the system at the infrastructure (I) level include Platoon Attack, Repudiation Attack, and Unauthorized Access etc.
    \item \textbf{Sensor-Based Attack:} These attacks concern about compromising the authenticity and availability of sensors over the vehicles including Illusion Attack, and Jamming Attack etc.
    \item \textbf{Wireless Communication-Based Attack:} These attacks focus on exploiting vulnerabilities within the communication protocols and channels, which are one of the most vulnerable targets in a vehicular network, such as Spoofing Attack, Spamming Attack, and Denial of Service (DoS) etc.
\end{itemize}

In order to overcome the above security threats and attacks in vehicular networks, effective security
mechanisms should be designed to ensure the appropriate operation. The key security services are as confidentiality, availability, integrity, privacy, and trust.

\subsection{AI-based Security-persevering Methods}

To address these important security and privacy threats encountered in vehicular networks, a number of works have been carried out on these security mechanisms. With the advancements in machine learning and deep learning technologies, AI-based methods have achieved significant success in security solutions
for vehicular networks. In the content of security-persevering vehicular network, the primary AI-based methods employed are summarized as below:

\begin{itemize}
    \item \textbf{Attack Detection:} Vehicular demands highly-efficient, intelligent, and faster solutions when vehicular networks are subjected to attacks. AI-based methods aim to detect a variety of attacks through experience and shared information, thereby enhancing the security of the vehicular networks. For instance, to detect DDoS attacks for given conditions, AI-based methods can be trained by ground truth data from transport control protocol (TCP) and user datagram protocol (UDP) in the presence as well as an absence of DDoS attacks. In case of an abnormality, it can be a classifier achieving excellent performance.
    \item \textbf{Intrusion Detection:} Intrusion detection system (IDS), or call misbehavior detection system, is a method focusing on detecting an unknown type of attacks or misbehavior. AI-based methods are typically employed to detect the type of misbehavior or intrusion attack that can be launched by a dishonest node. These methods leverage artificial intelligence to analyze patterns, behaviors, and anomalies, enabling the identification of malicious activities and potentially harmful nodes within the vehicular network, thus enhancing overall network security and integrity.
    \item \textbf{Trust Computation:} Trust computation aim to ensure honesty among vehicular network and enhance the protection level of the system from attackers. AI-based methods identify honest and dishonest nodes or evaluate the trustworthiness of data transmitted between nodes. Several trust computation mechanism are proposed to access integrity and accuracy in event messages and their sender.
    \item \textbf{Privacy Protection:} Privacy protection aim to protect the sensitive information of vehicular network from attackers. It can be categorized into location privacy and user privacy. AI-based methods are mainly within the Federated Learning (FL) framework to share secure data. This approach is important for vehicular networks where preserving the confidentiality and integrity of the data is crucial while allowing collaborative learning and enhancements.
\end{itemize}


\subsection{Limitations of AI-based Methods}\label{Lim}

Even though AI-based methods have shown significant efficacy in preserving security, there still exist many limitations of them. Several limitations, such as Adversarial Attack, Energy Constraint, Latency Limitation, and Computation Cost etc, additionally intensify the trade-off between security-preserving and resource allocation in vehicular networks. 

In the content of security and privacy in AI-based methods, Adversarial Attack is a new type of attack focusing on the AI-based models. It aims to supply deceptive inputs to AI-based model and attempt to fool it. These kinds of specialized adversarial attacks against neural networks significantly impact the detection accuracy of AI-based methods, potentially leading to security breaches in vehicular networks, and even posing dangers to human safety. 

Therefore, deploying robust and reliable AI-based methods in security-sensitive vehicular networks is critically important.




==> Sensing.tex <==
\section{Sensing}

5G

Channel-aware adversarial attacks against deep learning-based wireless
signal classifiers,

How to attack and
defend 5G radio access network slicing with reinforcement learning

Adversarial machine learning for flooding
attacks on 5G radio access network slicing,

Adversarial attacks
on deep learning based mmWave beam prediction in 5G and beyond



\subsection{trust management systems}


\cite{yang2022generative} Generative Adversarial Learning for Trusted and Secure Clustering in Industrial Wireless Sensor Networks

\pending{

Abstract—Traditional machine learning techniques have
been widely used to establish the trust management systems.
However, the scale of training dataset can significantly
affect the security performances of the systems,
while it is a great challenge to detect malicious nodes due
to the absence of labeled data regarding novel attacks. To
address this issue, this article presents a generative adversarial
network (GAN) based trust management mechanism
for industrial wireless sensor networks. First, type-2 fuzzy
logic is adopted to evaluate the reputation of sensor nodes
while alleviating the uncertainty problem. Then, trust vectors
are collected to train a GAN-based codec structure,
which is used for further malicious node detection. Moreover,
to avoid normal nodes being isolated from the network
permanently due to error detections, a GAN-based trust
redemption model is constructed to enhance the resilience
of trust management. Based on the latest detection results,
a trust model update method is developed to adapt to the
dynamic industrial environment. The proposed trust management
mechanism is finally applied to secure clustering
for reliable and real-time data transmission, and simulation
results show that it achieves a high detection rate up to
96%, as well as a low false positive rate below 8%.

}

However, the scale of training dataset can significantly
affect the security performances of the systems,
while it is a great challenge to detect malicious nodes due
to the absence of labeled data regarding novel attacks. To
address this issue, this article presents a generative adversarial
network (GAN) based trust management mechanism
for industrial wireless sensor networks.

\subsection{Intrusion Detection}


% \cite{zhou2020indoor} Indoor WLAN intelligent target intrusion sensing using ray-aided generative adversarial network

% \pending{

% However, the existing indoor
% WLAN target intrusion sensing approaches usually depend
% on the radio map construction with huge labor and time cost,
% which is the major barrier of current systems. In response to
% this compelling problem, we propose the new ray-aided generative
% adversarial model (RaGAM) to automatically construct the
% radio map, which is used for the indoor WLAN intelligent target
% intrusion sensing and localization.

% The paper introduces a novel ray-aided generative adversarial model (RaGAM) for automatic construction of radio maps used in WLAN-based target intrusion sensing and localization.
% It demonstrates the feasibility of using adaptive-depth ray tree-based quasi three-dimensional ray-tracing models for depicting WLAN signal variations.
% Incorporation of a modified Generative Adversarial Network (GAN) with joint synthetic and unsupervised learning improves the precision of the ray-tracing model.



% Type: Empirical study using a quasi 3D ray-tracing model and a modified GAN for radio map construction.
% Implications: Demonstrates the feasibility and efficiency of the proposed approach in practical settings.
% Reasoning: The approach is chosen to address the limitations of existing methods in terms of labor and time costs【8†source】【12†source】.


% List: The approach may have limitations in complex or varying environments and with multiple intrusion targets.
% Mitigations: Future research is suggested to address these limitations, including improving multi-target intrusion sensing and adapting to dynamic environments【24†source】.

% }



\cite{rathinavel2022efficient} Efficient Generative Wireless Anomaly Detection for Next Generation Networks

\pending{

The study introduces efficient methods for detecting anomalies in wireless signals using advanced machine learning techniques, enhancing security in next-generation networks.
In general, while looking at
raw spectrum data, some signal processing step is applied
to the data before it can be fed into the anomaly detection
model. This step is storage and computationally demanding.
Examples of such data include spectrogram of time-frequency
or spectral correlation function outputs [6] [7], power spectral
density data [8] [9] and dynamic spectrum access data [10]
[11]. Further, [12] [13] look at ML-based sensing of the air
interface, but they largely all rely on high-rate radio timeseries
sample data which is large and cumbersome to store
and/or transmit. Hence, although existing literature addresses
anomaly detection in wireless data, they are either storage or
compute-intensive or are very application specific.
In this work, we focus on a scalable solution to this problem,
which leverages metadata as its input for anomaly detection
which can be easily stored or transmitted, and which represents
a high-level summarization of activity in order to enable
downstream sense-making from numerous radios or sensors.

requiring significantly
less storage and/or bandwidth to process and act on
large spans of time and numbers of sensors.

Anomaly detection in wireless signals through multisensor
fusion has numerous real-world applications including
spectrum monitoring and awareness, fault detection, and spectrum security.

What is the primary challenge addressed in the paper?
The challenge is efficiently detecting anomalies in wireless signals in next-generation networks, crucial for security and spectrum management【33†source】.
How do the proposed methods contribute to wireless network security?
By detecting anomalies in wireless signals, the methods enhance the security and efficiency of spectrum management in next-generation networks like 5G and 6G【33†source】.
What makes this research significant in the context of current and future wireless networks?
The research is significant due to its application in enhancing the security and management of increasingly dense and complex wireless networks, including 5G and 6G【33†source】.

Goal: To develop efficient and scalable methods for anomaly detection in wireless signals for next-generation networks.
Research Questions/Hypotheses: Can advanced machine learning techniques effectively detect anomalies in wireless signals for enhanced security in next-generation networks?
Significance: The research addresses the critical need for robust security measures in increasingly complex wireless networks.

}


\cite{cheng2022resnet} ResNet-AE for Radar Signal Anomaly Detection

\pending{

Radar signal anomaly detection is an effective method to detect potential threat targets.

In 2018, Xu et al. constructed
the donut algorithm [12] based on the VAE, which trains the normal and abnormal
data simultaneously, making the feature extraction more complete and providing a new
idea for the VAE-based anomaly detection algorithm. In 2019, Chen et al. used the confrontational
training method, Buzz [13], to detect anomalies in complex time series. This
method not only reached a very high level in the public dataset but also gave a theoretical
inference to transform the model into a Bayesian network, which enhanced the interpretability
of the model. In 2020, Niu et al. proposed a VAE-GAN detection model [14]. The model
jointly trains the encoder, generator, and discriminator, which can improve the fidelity of
signal reconstruction, make the distinction between normal and anomalies more significant,
and improve anomaly detection Accuracy. Lin et al. proposed a mixed anomaly detection
method [15], which combines the representation learning ability of the VAE with the time
modeling ability of the LSTM. The VAE structure aims to capture the structural rules of
the time subsequence on the local window, while the LSTM structure models the changing
trend of the long-term time series. Audibert et al. proposed a fast and stable unsupervised
anomaly detection method, USAD, for multivariate time series [16]. This method uses the
automatic encoder architecture to meet the conditions of unsupervised learning. The use of
adversarial training enables rapid training and the isolation of anomalies. Experiments on
five public and proprietary datasets verify its high robustness, training speed, and anomaly
detection performance. Huang et al. proposed an unsupervised time-series anomaly detection
method based on multimodal countermeasure learning [17], which converts the
original time series into frequency-domain space, constructs a multimodal time series
representation, uses a multimodal generation countermeasure network model, and realizes
unsupervised joint learning of normal time-series information about time-domain and
frequency-domain feature distribution for multimodal time series, The anomaly detection
problem is transformed into the measurement problem of time-series reconstruction in
time-frequency space. The anomaly of time series is measured from the time domain and
frequency domain. Compared with the traditional single-mode method, this method has
improved the AUC and AP by 12.50% and 21.59%, respectively, which provides a new
direction for electromagnetic signal anomaly detection based on deep learning.
However, GAN networks tend to have complex structures and a high overhead of
training and detection, while traditional AE networks have low Accuracy in anomaly
detection of electromagnetic signals. Therefore, this paper proposes a ResNet-AE network
model based on the AE network. This model uses the encoder and decoder with ResNet
for feature mapping and data reconstruction. It can effectively alleviate the problem of
gradient disappearance, improve the depth of the network that can be effectively trained,
and improve the ability of network feature extraction and reconstruction. LSTM is used to
acquire time-dependent features. Cluster analysis is used to process the anomaly detection
results to obtain an adaptive decision threshold.

}



\cite{harini2023data} Data Anomaly Detection in Wireless Sensor Networks Using $\beta$-Variational Autoencoder

\todo{Data imbalance }

\pending{

Data imbalance is the major challenge in
machine learning models that is resolved in the proposed model
using deep learning technique.

AD becomes a major challenge in Wireless Sensor networks
in order to reduce false alarms[12]. Sensors generate sensory
data and continuously monitor physical factors including
temperature, vibration, and motion. A sensor node may act as
a data router and data originator simultaneously. On the other
hand, a sink acts as the center of processing and gathers data
from sensors. To share data, the base station of a Wireless
Sensor Networks(WSN) system makes a connection to the
Internet.

β-VAEs learn a disentangled representation of a data
distribution; that is, a single unit in the latent code is only
responsive to a single generating element. The benefit of using
a disentangled representation is that the model is
straightforward to generalize and interpret. For the loss
function, beta divergence is employed instead of KL
divergence as in [1]. The purpose for adding this hyper
parameter is to optimize the likelihood of generating a true
dataset while decreasing the likelihood of real to estimated
data being minimal, under epsilon.

Takeaways:
The β-Variational Autoencoder (VAE) effectively addresses data imbalance and detects anomalies in wireless sensor networks.
The introduction of the β parameter to the VAE's loss function provides a disentangled representation of data.
The model uses multivariate normal distribution for anomaly detection, which is particularly effective in imbalanced datasets.
Practical Implications: The approach can be implemented in various IoT and sensor network settings for enhanced anomaly detection.
Potential Impact: Could lead to more robust and efficient security systems in wireless sensor networks.

Model Complexity and Computational Resources: The implementation of β-Variational Autoencoders, being a deep learning model, might require significant computational resources. This could be a limitation in scenarios where sensor nodes have limited processing capabilities or in large-scale deployments where computational efficiency is critical.

Data Preprocessing Requirements: The methodology requires thorough data preprocessing, including the elimination of rows with NaN values and the transformation of arrays into tensors. This preprocessing step could be challenging in real-time applications where data is continuously streamed from sensors.

Fixed Threshold for Anomaly Classification: The paper sets a threshold for anomaly classification based on the maximum of the average losses of each batch. This fixed threshold approach might not be adaptable to different or changing environmental conditions, potentially affecting the model's accuracy in diverse scenarios.

Testing with Synthetic Anomalies: The testing phase involves introducing synthetic outliers into the dataset. While this approach is practical for evaluation, it might not fully replicate the complexity and unpredictability of real-world anomalies.

Generalization to Different Types of Sensor Data: The paper primarily focuses on specific datasets (IBRL and ISSNIP). It's unclear how well the model generalizes to other types of sensor data or different sensor network configurations.

Real-Time Processing Capabilities: The model's ability to process data in real-time and adapt to immediate changes in the sensor environment is not explicitly addressed. This is crucial for many applications of wireless sensor networks.

Scalability: The scalability of the approach to larger and more complex wireless sensor networks is not thoroughly explored. This is particularly important for IoT applications where networks can be extensive and diverse.

}


\cite{luo2018distributed} Distributed Anomaly Detection using Autoencoder Neural Networks in WSN for IoT

\pending{

In reality, however, such signals
or data are rarely perfect, where anomalies often arise and
can interfere with the subsequent IoT analytics. Anomalies,
also known as outliers, are data that do not conform to
the patterns exhibited by the majority of the data set

Wireless sensor networks (WSN) are fundamental
to the Internet of Things (IoT) by bridging the gap between the
physical and the cyber worlds.

Anomaly detection is a critical
task in this context as it is responsible for identifying various
events of interests such as equipment faults and undiscovered
phenomena.

Introduction of autoencoder neural networks in wireless sensor networks (WSN) for IoT improves anomaly detection.
A two-part algorithm is designed, minimizing communication overhead and computational load on sensors.
Demonstrated high detection accuracy and low false alarm rate in a real-world testbed.
The system is capable of adapting to new changes in a non-stationary environment.

What is the primary innovation of the research?
The primary innovation is the introduction of autoencoder neural networks into WSN for IoT, specifically for distributed anomaly detection【54†source】.
How does the proposed system work?
The system uses a two-part algorithm that allows for anomaly detection at sensors in a fully distributed manner without the need for extensive communication with other sensors or the cloud【55†source】.
What are the benefits of this approach?
The approach minimizes communication overhead and computational load on sensors, making it suitable for resource-limited environments like WSN【55†source】.

List: Possible limitations in detecting certain types of anomalies or in complex IoT environments.
Mitigations: Suggests future work to enhance the models and explore additional features for anomaly detection.

}


\cite{hasan2023wasserstein} Wasserstein GAN-based Digital Twin Inspired Model for Early Drift Fault Detection in Wireless Sensor Networks

\todo{

In very recent times, a new method for fault or anomaly
detection has been applied by constructing the digital equivalent
of a physical system [40]. This approach involves a digital
representation of the underlying system, which is termed a
digital twin (DT) that usually simulates normal operating
behavior. Deciding on the occurrence of a fault is made when
the residual between the signal obtained from the DT and the
real-measured signal exceeds a defined threshold. Construction
of the DT is often based on the physical laws on which
a particular component of a system operates. As in [41],
a DT estimator of a photovoltaic energy conversion unit is
developed. The design of the estimator for a single-energy
conversion unit involves convoluted modeling steps. In [42]
a DT-based fault detection is proposed for bearing fault
detection. Also, in this case, the authors combine signal
approximation and signal estimation stages to create a DT.
Both the approximation and estimation stages have several
complex subsystems. It is evident that this approach gets
severely complex and is error prone when the system under
consideration consists of a number of subsystems, in which
responses depend on each other. However, using DNNs to
generate DTs has recently been tapped by some researchers.
A relatively new concept is the generative adversarial network
(GAN) approach, which seems promising for creating DTs.
The capability of generating artificial samples very similar
to the training examples provided is the key idea behind
creating DTs using GANs. Xu et al. [43] proposed an anomaly
detection framework based on a DT, where the DT is created
from a GAN architecture. The generator segment is composed
of a graph convolutional network (GCN), a polling layer, and
LSTM layers, and the discriminator segment is a multiclass
classifier. A conditional-style GAN architecture was presented
in [44] to create a DT for a machining model that generates
time-series data representing a vibration signal. Booyse et al.
demonstrated that DTs based on deep generative models can
be used in fault detection and analysis [45].

}


\pending{

Based on the data from these devices, numerous
services and systems are now offered where critical
decisions depend on the data collected by sensors. Therefore,
error-free data are most desirable, but due to extreme
operating environments, the possibility of faults occurring
in sensors is high. So, detecting faults in data obtained
by sensors is important.

"The proposed model is not a complete DT but is inspired by the DT's ability to mimic the physical system."
"The discriminator segment of the trained GAN model is used for fault detection."
"The best fault detection accuracy achieved by the proposed model is 98.7%."

Q: What is the main objective of the proposed model? A: To detect drift faults in sensor data in wireless sensor networks.
Q: How does the model achieve fault detection? A: By using a Wasserstein GAN-based digital twin model that mimics the normal state of a sensor.
Q: What level of accuracy does the model achieve? A: The model achieves a fault detection accuracy of up to 98.7%.

We developed a virtual sensor motivated by the DT concept
using the Wasserstein GAN (WGAN) architecture.
We demonstrated that with this GAN model, the normal
operating behavior of a physical sensor can be realized.

List: Limited to the detection of drift faults; may not generalize to other types of sensor faults.
Mitigations: Future work could explore the model's applicability to other fault types.

}


% \cite{lu2021gan} GAN-based data augmentation strategy for sensor anomaly detection in industrial robots

% \cite{xie2020unsupervised} Unsupervised deep spectrum sensing: A variational auto-encoder based approach

% \pending{

% }


\cite{rubio2023intelligent} Intelligent Sensing and Learning for Advanced MIMO Communication Systems


\cite{ding2024gan} A GAN-based security strategy for WSN networks based on honeypot algorithm
(strategy)

\pending{

Owing to constrained resourceof sensor nodes, a significant level of
redundancy, network data’s higher correlation,intrusion detection schemes for wireless sensor networks also
have the drawbacks ofpoor identification rate, high computation overhead, and higher false alarm rate.

Tooverwhelm
the above problems, in this manuscript, Self-Attention-Based ProvisionalVariational Auto-Encoder
Generative Adversarial Network (SAPVAGAN) optimized withHoney Badger Algorithms proposed for
enhancing Cyber security in Wireless sensornetwork(ECS-WSN-SAPVAGAN–HBA).

Based on the optimum features,
the intruders in WSN data are categorizedinto normal and anomalous data (Black hole attack, Gray hole
attack, Flooding attackand Scheduling attacks) with the help of SAPVAGAN.In general, SAPVAGANnotexpose
any adaption of optimization modes for determining better parameters toassure accurate detection of WSN
intrusion.

Takeaways:
The SAPVAGAN optimized with Honey Badger Algorithm (ECS-WSN-SAPVAGAN-HBA) effectively detects intrusions in WSNs.
The use of GAN (Generative Adversarial Network) and Honey Badger Algorithm enhances the accuracy of intrusion detection.
This method shows significant improvements over existing methods in terms of prediction accuracy and sensitivity.
Practical Implications: The strategy can be applied in diverse WSN applications for more secure and reliable operations.
Potential Impact: Could set a new standard for intrusion detection in WSNs, influencing future cybersecurity strategies.


Unfortunately, gives a major challenge achieve this objectives in the
unnatural resources ofWSNs together with storage,rectifying capacity
and battery energy [5,6]. Such features givestraditional safety measures
such cryptography not always enough like networks [7]. WSNsare very
exposed the possibility of being attacked, due to their unlocked and
shared natureand small materials of the detector nodes

Existing methods for intrusion detection increase time consumption
while also not offeringhigh accuracy and detection rates. Some conventional
network intrusion detection techniquesare no longer useful
since WSNs differ from typical computer networks in many ways,
including terminal kinds, data transfer, network topology, and a number
of other areas. IDSmust be highly accurate when identifying intruders,
involving unknown attacks, itwellsituatedto make sure low overhead in
WSN communication. These are the two keyrequirements when creating
IDS for WSN. Hence, in this manuscriptSAPVAGANoptimizedwith
Honey Badger Algorithm is proposed for intrusion detection scheme
whichconform theproperties of WSN.

"Owing to constrained resource of sensor nodes, intrusion detection schemes for wireless sensor networks also have the drawbacks of poor identification rate, high computation overhead, and higher false alarm rate"【98†source】.
"The proposed ECS-WSN-SAPVAGAN–HBA method is performed in Python utilizing the WSN-DS dataset"【98†source】.
"The performance of the proposed ECS-WSN-SAPVAGAN-HBA method provides higher prediction accuracy" compared with existing methods【106†source】.


List: Specific limitations are not detailed in the quoted sections, but potential limitations could include the complexity of the method, computational resource requirements, and the need for specialized knowledge for implementation.
Mitigations: Not discussed in the document.

}

\cite{lin2023physical} Physical Layer Security Enhancement in Energy Harvesting-based Cognitive Internet of Things: A GAN-Powered Deep Reinforcement Learning Approach

\pending{

Cognitive Radio (CR) is regarded as the key technology
of the 6th-Generation (6G) wireless network. Because
6G CR networks are anticipated to offer worldwide coverage,
increase cost efficiency, enhance spectrum utilization, improve
device intelligence and network safety. This paper studies the
secrecy communication in an Energy Harvesting (EH)-enabled
Cognitive Internet of Things (EH-CIoT) network with a cooperative
jammer. The Secondary Transmitters (STs) and the
jammer first harvest the energy from the received Radio Frequency
(RF) signals in the EH phase. Then, in the subsequent
Wireless Information Transfer (WIT) phase, the STs transmit
secrecy information to their intended receivers in the presence
of eavesdroppers while the jammer sends the jamming signal
to confuse the eavesdroppers. To evaluate the system secrecy
performance, we derive the instantaneous secrecy rate and the
closed-form expression of Secrecy Outage Probability (SOP).
Furthermore, we propose a Deep Reinforcement Learning (DRL)-
based framework for the joint EH time and transmission power
allocation problems. Specifically, a pair of ST and jammer over
each time block is modeled as an agent which is dynamically
interacting with the environment by the state, action and reward
mechanisms.

Fortunately, Cognitive Radio (CR) has been considered as
an intelligent and promising technology to address spectrum
demands of wireless network by allowing Secondary Users
(SUs) to access the licensed spectrum bands owned by the
Primary Users (PUs) without causing harmful interference
to PUs [5].wind, thermal, vibration and Radio Frequency (RF) signals
[11]. Compared with harvested energy from natural energy
sources, the energy harvested from RF sources are more stable
and sustainable since RF signals can be continuously acquired
from the surrounding transmitters [12]. By combining the EH
technology with the CIoT system, the EH-enabled CIoT (EHCIoT)
has been proven to have excellent performances, for
instance, [7] proposed two Simultaneous Wireless Information
and Power Transfer (SWIPT) cooperative spectrum sharing
schemes to improve the energy and spectrum efficiency for
6G-enabled CIoT systems.

We consider an EH-CIoT system where the communication
security of the SU network is under threat
and thus a cooperative jammer is deployed for secure
wireless transmissions. We analyze and formulate two
optimization problems to maximize the average minimum
secrecy rate and to minimize the average maximum SOP
by considering some requirements, such as transmission
power, QoS and energy causality constraints. The purpose
of this paper is to enhance PLS by achieving the optimal
resource allocation for our proposed problems on secrecy
communication.

Takeaways: Demonstrates the effectiveness of combining Deep Reinforcement Learning with GANs for optimizing resource allocation in EH-CIoT systems to enhance security.
Practical Implications: Offers a viable solution for improving secrecy rates and reducing secrecy outage probability in wireless networks.
Potential Impact: Could significantly contribute to the development of more secure and efficient wireless communication systems.

"To evaluate the system secrecy performance we derive the instantaneous secrecy rate and the closed-form expression of Secrecy Outage Probability (SOP)."
"A pair of ST and jammer over each time block is modeled as an agent dynamically interacting with the environment by the state action and reward mechanisms."
"The simulation results show that our proposed method is highly effective in maximizing the secrecy rate while minimizing the SOP compared with other existing schemes."

What is the main focus of the paper?
Enhancing physical layer security in EH-CIoT networks using a GAN-powered DRL approach.
How does the proposed system work?
It uses DRL for joint EH time and transmission power allocation, with LSTM and GAN for optimal solutions.
What are the key benefits of this approach?
Maximizes secrecy rate and minimizes SOP effectively compared to other methods.

List: Potential limitations in real-world implementation, complexity of the DRL framework.
Mitigations: The paper suggests further research for practical applications.



}


% \cite{shahid2021data} Data-driven Approach Based on Deep Learning and Probabilistic Models for PHY-layer Security in AI-enabled Cognitive Radio IoT.

% \cite{nooraiepour2023novel} Novel Enabling Components for Physical Layer Security Powered by Deep Learning Algorithms and Metamaterial Antennas




\subsection{Data Augmentation}

\todo{Activity Recognition (High probability omit)}

\cite{yun2023gan} GAN-based sensor data augmentation: Application for counting moving people and detecting directions using PIR sensors

? \cite{mehta2023deep} Deep Learning Techniques for Radar-Based Continuous Human Activity Recognition


\cite{qu2021wgan} WGAN-GP-based synthetic radar spectrogram augmentation in human activity recognition


\cite{subray2021towards} Towards enhancing spectrum sensing: Signal classification using autoencoders

\cite{vishwakarma2021gan} Gan based noise generation to aid activity recognition when augmenting measured wifi radar data with simulations

\pending{

Activity Recognition

}




